OneFlow: Redesign the Distributed Deep Learning Framework from Scratch

Deep learning frameworks such as TensorFlow and PyTorch provide a productive interface for expressing and training a deep neural network (DNN) model on a single device or using data parallelism. Still, they may not be flexible or efficient enough in training emerging large models on distributed devices, which require more sophisticated parallelism beyond data parallelism. Plugins or wrappers have been developed to strengthen these frameworks for model or pipeline parallelism, but they complicate the usage and implementation of distributed deep learning. Aiming at a simple, neat redesign of distributed deep learning frameworks for various parallelism paradigms, we present OneFlow, a novel distributed training framework based on an SBP (split, broadcast and partial-value) abstraction and the actor model. SBP enables much easier programming of data parallelism and model parallelism than existing frameworks, and the actor model provides a succinct runtime mechanism to manage the complex dependencies imposed by resource constraints, data movement and computation in distributed deep learning. We demonstrate the general applicability and efficiency of OneFlow for training various large DNN models with case studies and extensive experiments. The results show that OneFlow outperforms many well-known customized libraries built on top of the state-of-the-art frameworks. The code of OneFlow is available at: https://github.com/Oneflow-Inc/oneflow.

==> SBPandAutoParallel.tex <==
\section{Auto-Parallel}\label{sec:auto-parallel}

SBP signature benefits users and developers by enabling them to configure parallelism easily by writing it in the configuration instead of dealing with all those MPI tools \cwu{clarify what those tools are} and worrying about load balance\cwu{not clear how SBP naturally resolve load balancing}. However, users still need to specify the SBP signature for each operator, which requires massive repetitive and empirical labor. It is shown that the problem of generating an operator-wise parallelism strategy for optimal performance is NP-hard\cite{kennedy1998automatic, chen1989index, li1991data}.

Jia proposes a dynamic programming algorithm to address this problem \cite{jia-2018-icml}. However, his algorithm only works for a mostly linear graph of operators \cite{wang-2019-eurosys} and might crash \cwu{crash or takes very long time} for a complex graph since it enumerating all possible candidates to look for an optimal strategy. We take the idea of node and edge elimination from \cite{jia-2018-icml} and generalize it.

In this section, we introduce our auto-parallel algorithm, which addresses the NP-hard problem for any complex graph. We design 4 graph reductions to iteratively simplify the graph and further search for a sub-optimal strategy in the pruned state space. We shall introduce the whole work-flow of our auto-parallel algorithm in 4 stages.


\subsection{Cost Model}
In this stage, we build a cost model to evaluate the runtime for computation and data transfer. The cost model is an undirected graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, converted from the directed acyclic computation graph, which keeps the original nodes and edges. Each node represents a operator and each edge represents the data transition between operators. We omit the direction of edges in $\mathcal{E}$ for generalization of all the eliminations in graph simplification.

\cwu{in the following paragraph, not clear how exactly the costs are being estimated.}
Each node is assigned to a set of SBP signature candidates that represents the possible configuration of parallelism strategy at this operator. We assign computation cost at nodes and copy cost on edges. Computation cost, denoted by $C_{n}(n_{i}, s_{i})$, is a number to estimate the execution time of current operator $n_{i}$ with strategy $s_{i} \in \mathcal{S}_{i}$, where $\mathcal{S}_{i}$ is the set of SBP signatures of $n_{i}$. We require a priori estimate which takes time complexity of current operator and running speed of different devices into account. Copy cost, denoted by $C_{e}(e_{i}, s_{j}, s_{k})$ is a number to estimate the communication time when transferring one tensor  \cwu{what is it?}  from an upstream operator $n_{j}$ to a downstream operator $n_{k}$, where $e_{i}=(n_{j}, n_{k})\in\mathcal{E}$. It is a priori estimate which takes the amount of transferred data and communication bandwidth between devices into account.

The state space of the possible combinations of SBP signatures over all nodes has a size of $\mathcal{O}(\prod_{n\in \mathcal{V}}{|\mathcal{S}_n|)})$ which is the product of the size of possible signatures over all nodes.

The cost model depends on the assumption that execution of different operators and data transition do not happen simultaneously \cwu{not clear why the cost models need to rely on this assumption}, which might not always be the case in practice. In our framework, we can start the computation of this operator while the upstream operator is throwing data to another downstream operator. Nevertheless, our auto-parallel algorithm still brings a great improvement in practice and further improvement will be performed in the future. Under this assumption, our goal is to minimize the total cost to get an effective configuration of SBP signatures.

\subsection{Graph Simplification}
\yipeng{There should be some figures in this section.}
After initialization, we get a cost model with a huge state space. We aim to simplify the topology and reduce state space of the model without losing the optimal strategy. To achieve this goal, we introduce node, edge, leaf elimination and node merging procedures.

\yipeng{Might delete node and edge elimination and quote paper from Jia Zhihao. Only show the difference.}

\paragraph{Node Elimination} Denote $deg(n_{i})$ by degree of node $n_{i}$, the number of nodes adjacent to $n_{i}$. If a cost model graph $\mathcal{G}$ includes a node $n_{i}$ with $deg(n_{i})=2$, then a node elimination replaces $n_{i}$ and its only two edges $e_{j}=(n_{i}, n_{j})$ and $e_{k}=(n_{i}, n_{k})$ with a new edge $e_{i}'=(n_{j}, n_{k})$. We choose a strategy $s_{i}$ that minimize the total cost for every possible combination of $s_{j}$ and $s_{k}$.
\begin{equation*}
    C_{e}(e_{i}', s_{j}, s_{k}) = \min_{s_{i}}\{C_{n}(n_{i}, s_{i}) + C_{e}(e_{j}, s_{i}, s_{j}) + C_{e}(e_{k}, s_{i}, s_{k})\}.
\end{equation*}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/node_elimination.eps}
        \caption{Node}.
        \label{figure:node elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/edge_elimination_v2.eps}
        \caption{Edge}.
        \label{figure:edge elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/leaf_elimination_v2.eps}
        \caption{Leaf}.
        \label{figure:leaf elimination}
    \end{subfigure}
    \caption{Elimination}

\end{figure}

\paragraph{Edge Elimination} If a cost model graph $\mathcal{G}$ includes multiple edges $e_{i}, 1\leq i \leq m$ with the same vertices $n_{1}, n_{2}$, then an edge elimination merges them into a new edge $e'=(n_{1}, n_{2})$. For any strategy combination $s_{1}, s_{2}$ of vertices $n_{1}, n_{2}$,
\begin{equation*}
    C_{e}(e', s_{1}, s_{2}) = \sum_{i=1}^{m}C_{e}(e_{i}, s_{1}, s_{2}).
\end{equation*}

\paragraph{Leaf Elimination} If a cost model graph $\mathcal{G}$ includes a node $n_{i}$ with $deg(n_{i})=1$, then a leaf elimination replaces $n_{i}, n_{j}$ and the only edge $e_{i}=(n_{i}, n_{j})$ connected to $n_{i}$ with a new node $n_{j}'$. We choose strategy $s_{i}$ to minimize the total cost for every possible strategy candidate of $s_{j}$.
\begin{equation*}
    C_{n}(n_{j}', s_{j}) = C_{n}(n_{j}, s_{j}) + \min_{s_{i}}\{C_{e}(e_{i}, s_{i}, s_{j}) + C_{n}(n_{i}, s_{i})\}
\end{equation*}

\paragraph{Node Merging} If a cost model graph $\mathcal{G}$ contains at least 4 nodes and it can not perform any of those eliminations,
$$\text{i.e. } deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G},$$
then it will either perform a node merging or terminate the simplification procedure. From all node pairs that the product of the number of their strategy candidates is less than or equal to a threshold $\alpha$, a node merging picks the one $(n_{i}, n_{j})$ with the largest common neighborhood, and then merges them into a new node $n'$, where the neighborhood of a node $n$ is defined by the set $\{n\}\cup\{n_{i}| \exists e=(n_{i},n)\in \mathcal{G}\}$.

We introduce a threshold $\alpha$ to avoid unlimited node merging and concentrating all the possible strategy into one node. Without the threshold, the number of possible strategies for the final node is as large as the whole state space and it will run out of memory before you get the final node.

We take the Cartesian product of strategy candidate set of $n_{i}$ and $n_{j}$ as the strategy candidate set of the new node $n'$, $\mathcal{S}' = \mathcal{S}_{i} \times \mathcal{S}_{j}$. We apply pruning operations by reducing impossible combinations of $s_{i}$ and $s_{j}$. For example, if we require an upstream operator and a downstream operator to share the same memory for a tensor, then we will cross out those combinations with different strategies of parallelism for that tensor.
\begin{equation*}
\begin{split}
    \forall s'=(s_{i}, s_{j}&) \in \mathcal{S'},\\
    C_{n}(n', s') =& C_{n}(n_{i}, s_{i}) + C_{n}(n_{j}, s_{j}) + \\
    &\left\{
    \begin{array}{ccl}
    0 & & {\text{if edge } (n_{i},n_{j})\notin \mathcal{G}} \\
    C_{e}(e, s_{i}, s_{j}) & & {\exists e=(n_{i}, n_{j})\in \mathcal{G}}
    \end{array}\right.
    \end{split}
\end{equation*}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/node_merge.eps}
    \caption{Node Merging}
    \label{fig:node merging}
\end{figure}

If any two nodes in $\mathcal{G}$ have a product of the number of strategy candidates greater than $\alpha$, we terminate the graph simplification and move on to the next stage.

\begin{table}[]
    \centering
    \begin{tabular}{|p{0.24\linewidth}|p{0.18\linewidth}|p{0.18\linewidth}|p{0.18\linewidth}|}
    \hline
       procedure & number of eliminated nodes & number of eliminated edges & complexity \\
       \hline
        \makecell[c]{Node \\ Elimination}  & 1 & 1 & $O(M^{3})$ \\
        \hline
        \makecell[c]{Edge \\ Elimination} & 0 & $k\geq 1$ & $O(kM^{2})$ \\
        \hline
        \makecell[c]{Leaf \\ Elimination}  & 1 & 1 & $O(M^{2})$ \\
        \hline
        Node Merging  & 1 & $k\in \{0, 1\}$ & $O(M^{2})$ \\
        \hline
    \end{tabular}
    \caption{Simplification Procedures Features}
    \label{tab:Elimination Complexity}
\end{table}

We list the time complexity for one step of elimination or merging in table \pageref{tab:Elimination Complexity}, where $M=\max \{|\mathcal{S}_{i}|, \alpha\}$ is the maximum number of strategy candidates while iteratively updating $\mathcal{G}$.

\subsection{Strategy Search}
After simplification of cost model, we get either a simple node or a new graph $\mathcal{G'}$ with $deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G'}$ and the average number of strategy candidates is greater than or equal to $\sqrt{\alpha}$.

If we get a simple node $n_{1}$ as the whole graph, then we simply choose the strategy with the smallest computation cost $C_{n}(n_{1}, s_{1})$.

Otherwise, we apply a greedy strategy search algorithm to find a sub-optimal solution.

First, we initialize all nodes with a random strategy and put all edges into a set $\mathcal{A}$. We repeat the adjustment procedure until $\mathcal{A}=\emptyset$.

During each iteration of adjustment, we take one edge $e=(n_{i}, n_{j})$ out from $\mathcal{A}$, traverse through every possible combination of strategies and find the one that minimize the total cost of graph $\mathcal{G'}$, denoted by $(s_{i}^{1}, s_{j}^{1})$. To minimize the total cost of graph, we only need to minimize the summery of the computation cost and the copy cost of the neighborhood of $n_{i}$ and $n_{j}$.
\yipeng{To speed it up, we store the summery of computation and copy cost of the neighborhood of $n_{i}$ and $n_{j}$  under different strategies $s_{i}, s_{j}$ into two temporary arrays separately.}
If the origin strategy combination $(s_{i}^{0}, s_{j}^{0})$ is different from $(s_{i}^{1}, s_{j}^{1})$, set the strategy at $n_{i}, n_{j}$ to be $s_{i}, s_{j}$ and then put all the edges in the neighborhood of $n_{i}, n_{j}$ in the set $\mathcal{A}$. Finally, we remove $e$ from $\mathcal{A}$ and move on to the next adjustment.
\yangfei{This paragraph is not readable, maybe there are some mistakes.}

\subsection{Backtracking}
\cwu{not clear what this backtracking is indeed doing} In the last stage, we have a simplified graph $\mathcal{G'}$ in which each node is assigned with a strategy. We need to use the information that we store during graph simplification to backtrack the strategies at nodes in the original graph $\mathcal{G}$. Then we can export those SBP strategies corresponding to each operator for further processing such as tensor shape computing under given parallelism strategy.


==> auto_parallel.tex <==
%\section{Static Scheduling}
\vspace{-0.4cm}
\section{Optimizing the Parallel Strategy}\label{sec:auto-parallel}
\vspace{-0.3cm}

SBP signature enables users to configure parallelism policy easily. However, users still need to specify the SBP property for each operator. A user-friendly framework should automate the process of inferring SBP property. Nevertheless, it is shown that the problem of generating an operator-wise parallelism strategy for optimal performance is NP-hard\cite{kennedy1998automatic, chen1989index, li1991data}. Jia proposes a dynamic programming algorithm to address this problem \cite{jia-2018-icml}. However, the algorithm only works for a mostly linear graph of operators \cite{wang-2019-eurosys} and might take too long to find a solution for a complex graph since it enumerates all possible candidates to look for an optimal strategy. We improve Jia's approach in several ways to handle a complex graph. The approach follows the workflow described in \cite{jia-2018-icml}, that is, building a cost model, performing graph simplification and searching. In the following, we just highlight the major improvements.

\vspace{-0.4cm}
\paragraph{Cost model construction} In \SysName{}, the cost model is an undirected graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, converted from the directed acyclic computation graph, which keeps the original nodes and edges. We find that omitting the direction of edge $\mathcal{E}$ helps perform various types of eliminations in graph simplification procedure. We assign computation cost at nodes to estimate the execution time of operators and communication cost on edges to estimate the time to transfer tensors.

\vspace{-0.4cm}
\paragraph{Graph simplification} After getting a cost model with a huge state space, we simplify the topology and reduce the state space without losing the optimal strategy. To achieve this goal, we use node, edge and leaf elimination approaches as shown in Figure \ref{figure:leaf elimination} and a node merging procedures as shown in Figure \ref{fig:node merging}. Node and edge elimination is generalized from \cite{jia-2018-icml} except that our node elimination is suitable for more cases since we omit the direction of edges.

Leaf elimination has not been used in the previous work. If a cost model graph $\mathcal{G}$ includes a node $n_{i}$ with $deg(n_{i})=1$, leaf elimination replaces $n_{i}, n_{j}$ and the only edge $e_{i}=(n_{i}, n_{j})$ connected to $n_{i}$ with a new node $n_{j}'$.

When a cost model graph $\mathcal{G}$ contains at least 4 nodes and it is not applicable to any of the above eliminations,
$\text{i.e. } deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G},$
it will either perform a node merging or terminate the simplification procedure. We introduce a threshold of strategy number at nodes to avoid unlimited node merging, which may lead to an exponential increasing in the number of possible strategies, and, as a result, running out of memory.

\vspace{-0.4cm}
\paragraph{Strategy search} After the simplification of the cost model, if we get a simple node $n_{1}$ as the whole graph, then we simply choose the strategy with the smallest computation cost. Otherwise, we will get a new graph $\mathcal{G'}$ with $deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G'}$. Then we apply a greedy search algorithm to find a sub-optimal solution. First, we initialize all nodes with a random strategy and put all edges into a set $\mathcal{A}$. We repeat the adjustment procedure until $\mathcal{A}=\emptyset$. During each iteration of adjustment, we take one edge $e$ out from $\mathcal{A}$, traverse through every possible combination of strategies and choose the one that minimizes the total cost of graph $\mathcal{G'}$. If the original strategy is different from the new one, we update all the edges connected to the node pair of $e$ in the set $\mathcal{A}$ and remove $e$ from $\mathcal{A}$. After the greedy search, we use the information that we store during graph simplification to backtrack and export the strategies at nodes in the original graph $\mathcal{G}$.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/node_elimination.eps}
        \caption{node $n_{i}$}
        \label{figure:node elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/edge_elimination.eps}
        \caption{edges $e_{1},e_{3}$}
        \label{figure:edge elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/leaf_elimination_v2.eps}
        \caption{leaf $n_{i}$}
        \label{figure:leaf elimination}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Three types of elimination operations to simplify the cost model graph.}
    \vspace{-0.3cm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/node_merge.eps}
    \vspace{-0.2cm}
    \caption{An example of node merging procedure.}
    \label{fig:node merging}
    \vspace{-0.5cm}
\end{figure}

\begin{comment}
SBP signature benefits users and developers by enabling them to configure parallelism easily by writing it in the configuration instead of dealing with all those MPI tools and worrying about load balance. However, users still need to specify the SBP signature for each operator, which requires massive repetitive and empirical labor. It is shown that the problem of generating an operator-wise parallelism strategy for optimal performance is NP-hard\cite{kennedy1998automatic, chen1989index, li1991data}.

Jia proposes a dynamic programming algorithm to address this problem \cite{jia-2018-icml}. However, his algorithm only works for a mostly linear graph of operators \cite{wang-2019-eurosys} and might crash for a complex graph since it enumerating all possible candidates to look for an optimal strategy.

In this section, we introduce our auto-parallel algorithm, which addresses the NP-hard problem for any complex graph. We design 4 graph reductions to iteratively simplify the graph and further search for a sub-optimal strategy in the pruned state space. We shall introduce the whole work-flow of our auto-parallel algorithm in 4 stages.


\paragraph{Cost Model}
In this stage, we build a cost model to evaluate the runtime for computation and data transfer. The cost model is an undirected graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, converted from the directed acyclic computation graph, which keeps the original nodes and edges. Each node represents an operator and each edge represents the data transition between operators.

Each node is assigned to a set of SBP signature candidates that represents the possible configuration of parallelism strategy at this operator. We assign computation cost at nodes to estimate the execution time of operators and communication cost on edges to estimate the communication time while transferring tensors between layers.

\paragraph{Graph Simplification}
After initialization, we get a cost model with a huge state space. We aim to simplify the topology and reduce the state space of the model without losing the optimal strategy. To achieve this goal, we introduce node, edge, leaf elimination and node merging procedures.

Node and edge elimination is generalized from \cite{jia-2018-icml} except that our node elimination is suitable for more cases since we omit the direction of edges.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/node_elimination.eps}
        \caption{Node}.
        \label{figure:node elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/edge_elimination.eps}
        \caption{Edge}.
        \label{figure:edge elimination}
    \end{subfigure}
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/leaf_elimination_v2.eps}
        \caption{Leaf}.
        \label{figure:leaf elimination}
    \end{subfigure}
    \caption{Elimination}

\end{figure}

If a cost model graph $\mathcal{G}$ includes a node $n_{i}$ with $deg(n_{i})=1$, then a leaf elimination replaces $n_{i}, n_{j}$ and the only edge $e_{i}=(n_{i}, n_{j})$ connected to $n_{i}$ with a new node $n_{j}'$. We choose strategy $s_{i}$ to minimize the total cost for every possible strategy candidate of $s_{j}$.

If a cost model graph $\mathcal{G}$ contains at least 4 nodes and it can not perform any of those eliminations,
$\text{i.e. } deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G},$
then it will either perform a node merging or terminate the simplification procedure. From all node pairs that the product of the number of their strategy candidates is less than or equal to a threshold $\alpha$, a node merging picks the one $(n_{i}, n_{j})$ with the largest common neighborhood, and then merges them into a new node $n'$.

We take the Cartesian product of strategy candidate set of $n_{i}$ and $n_{j}$ as the strategy candidate set of the new node $n'$, $\mathcal{S}' = \mathcal{S}_{i} \times \mathcal{S}_{j}$. We apply pruning operations by reducing impossible combinations of $s_{i}$ and $s_{j}$.

We introduce a threshold $\alpha$ to avoid unlimited node merging, which leads to an exponential increase in the number of possible strategies and, as a result, running out of memory.


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/node_merge.eps}
    \caption{Node Merging}
    \label{fig:node merging}
\end{figure}

If any two nodes in $\mathcal{G}$ have a product of the number of strategy candidates greater than $\alpha$, we terminate the graph simplification and move on to the next stage.

\paragraph{Strategy Search}

After simplification of the cost model, if we get a simple node $n_{1}$ as the whole graph, then we simply choose the strategy with the smallest computation cost.

Otherwise, we will get a new graph $\mathcal{G'}$ with $deg(n_{i})  \geq 3, \forall n_{i}\in \mathcal{G'}$. Then we apply a strategy search algorithm to find a sub-optimal solution.

First, we initialize all nodes with a random strategy and put all edges into a set $\mathcal{A}$. We repeat the adjustment procedure until $\mathcal{A}=\emptyset$.

During each iteration of adjustment, we take one edge out from $\mathcal{A}$, traverse through every possible combination of strategies and choose the one that minimizes the total cost of graph $\mathcal{G'}$.
If the origin strategy combination is different from the new one, put all the edges connected to the node pair in the set $\mathcal{A}$. Finally, we remove $e$ from $\mathcal{A}$ and move on to the next adjustment.

\paragraph{Backtracking}
In the last stage, we have a simplified graph $\mathcal{G'}$ in which each node is assigned with a strategy. We use the information that we store during graph simplification to backtrack and export the strategies at nodes in the original graph $\mathcal{G}$ for further processing.

\end{comment}


==> depracated_evaluation.tex <==
\section{Deprecated Case Study and Evaluation}
\label{sec:deprecated_evaluation}

\begin{itemize}
    \item Pipelining in Nvidia Dali
    \item Pipelining parallelism in PipeDream
    \item support model parallelism (mesh-tensorflow, GShard, face, deep and wide, gpt-3)
    \item Gradient Accumulation
    \item Optimizer Placement Optimization (deepspeed)
    \chengcheng{Q: Is this list to be deleted in the final version? }
    \item support auto-parallelism (zhihao jia)
    \item Dynamic Loss Scaling
    \item Synchronous BatchNorm
    \item Parallel Softmax, demonstrate the SBP deduction
\end{itemize}

\chengcheng{We don't use auto-parallel in other case, like InsightFace, HugeCTR, etc. Should we explain that? And the key point of the experiment is to prove that \SysName{} supports all kinds of parallelism and cases more simply and efficiently. Should the number of code lines be compared with other frameworks like DeepSpeed, Megatron and PipeDream?}

We compare both the throughput and the memory footprint.

\yipeng{We need to specify the hardware condition. One example quoted from other paper:

All of our experiments use up to 32 DGX-2H servers (a total
of 512 Tesla V100 SXM3 32GB GPUs). Our infrastructure is optimized for multi-node deep learning applications,
with 300 GB/sec bandwidth between GPUs inside a server
via NVSwitch and 100 GB/sec of interconnect bandwidth
between servers using 8 InfiniBand adapters per server.}

\subsection{Auto-Parallel}

\jinhui{yinggang, yipeng, yangfei}
\jinhui{Please add experiments to demonstrate that the policy obtained by auo-parallel module is consistent with manual parallelism. Furthermore, it can discover better policy which has not been previously explored by experts. We can design an experiment setting, in which we fix the CNN backbone while gradually increase the size of fully connected layer. In the beginning, the optimal parallelism policies for both backbone and fully connected layer are data-parallelism. However, when the size of fully connected layer is sufficiently large, its optimal policy will become model parallelism.}

In this work, we conduct an experiment to compare the performance of data parallelism, model parallelism and auto parallelism on AlexNet. As known to all, AlexNet contains five convolutional layers followed by three fully connected layers. We control the parallelism strategy under configuration of data and model parallelism for those fully connected layers and compare the performance with our auto-parallel system. We train AlexNet with different batch size $b$ and number of classes $c$, which is number of columns in the weight tensor in the last layer.



Shown in figure [], model parallelism runs faster than data parallelism since we have 4096 neurons for two hidden layers with $b \leq 1024$. For such configuration, our auto-parallel system chooses model parallelism on the first two fully connected layers for any $b$ and $c$. As batch size increases, throughput rate increase and it turns to use hybrid parallelism for the last layer. It should become data parallelism when batch size is large enough. However, our machine is not supported to train an AlexNet with $b \geq 4096$. Still, we can visualize some speedup while using our auto-parallel system.

\subsection{Data Pre-processing Pipeline}

\jinhui{sunxue}
Data parallelism is widely used for scaling DNN training over large datasets, but mainstream deep learning frameworks usually pay most attention to optimize the intern computing primitives, not for the data layer, which is in charge of reading and preprocessing input data[].

Fundamentally current deep learning frameworks use a DAG model to delineate different algorithms to build networks, however, ignorance of data loading and preprocess means frameworks don't draw this into the computing graphs so that the whole data fetching will not be taken into consideration when optimizing or overlapping with other computing. It has exactly become the system bottleneck when input data is extremely increasing in amounts[].

Hence it could be easily inferred that properly reading and preprocessing input data will achieve expediting distributed DNN training performance if the overlap method works. We have picked ResNet50-v1.5[], one typical DNN network in NVIDIA implementation[], and have experimented by using synthetic data, which is kind of fake data generated by the memory and does not need to load via I/O devices when training, and real data on the disk.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/torch-syn-data-com.eps}
         \caption{}.
         \label{figure:torch_syn_data_com}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/tf-syn-data-com.eps}
         \caption{}.
         \label{figure:tf_syn_data_com}
     \end{subfigure}
     \caption{FP32 throughputs(samples/sec) of mainstream frameworks using synthetic data and real data}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/torch-syn-data-amp-com.eps}
         \caption{}.
         \label{figure:torch_syn_data_amp_com}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/tf-syn-data-amp-com.eps}
         \caption{}.
         \label{figure:tf_syn_data_amp_com}
     \end{subfigure}
     \caption{AMP throughputs(samples/sec) of mainstream frameworks using synthetic data and real data}
\end{figure}

Figure \ref{figure:torch_syn_data_com},\ref{figure:tf_syn_data_com} shows models training in each framework can get better throughputs when loading simulated synthetic data, compared with loading normal data which has to be transferred from the disk and carried to the GPUs with the original data loader. However when training with mixed-precision data (See Figure \ref{figure:torch_syn_data_amp_com}, \ref{figure:tf_syn_data_amp_com}), it exacerbates performance yet, because bits computed decrease brings about computation decrease, then data delivery still cannot catch up on the computation even in the NVIDIA-optimized frameworks.

In fact, it is, and that is why third party libraries, such as DALI, occurred to improve data loading ability for current frameworks that cannot handle it efficiently(See Figure \ref{figure:torch_data_dali_com}, \ref{figure:tf_data_dali_com}, \ref{figure:torch_data_dali_amp_com}, \ref{figure:tf_data-dali_amp_com}). 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/torch-data-dali-com.eps}
         \caption{}.
         \label{figure:torch_data_dali_com}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/tf-data-dali-com.eps}
         \caption{}.
         \label{figure:tf_data_dali_com}
     \end{subfigure}
     \caption{FP32 real data throughputs(samples/sec) of mainstream frameworks using its original loader and DALI}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/torch-data-dali-amp-com.eps}
         \caption{}.
         \label{figure:torch_data_dali_amp_com}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/tf-data-dali-amp-com.eps}
         \caption{}.
         \label{figure:tf_data-dali_amp_com}
     \end{subfigure}
     \caption{AMP real data throughputs(samples/sec) of mainstream frameworks using its original loader and DALI}
\end{figure}
 
Even so, a well-organized system design performs better than a plug-in integrated from the outside. So we propose a data pre-process pipeline implemented concisely with \SysName{} actor architecture(see Figure \ref{figure:data_loader_preprocess_in_xFlow}).

\begin{figure}
    \centering
     %\begin{subfigure}[b]{0.12\linewidth}
         \centering
         \includegraphics[width=1.5\linewidth]{figure/preprocess_timeline.eps}
         \caption{Data pipeline timeline in \SysName{} }.
         \label{figure:preprocess_timeline}
   %  \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     %\begin{subfigure}[b]{0.12\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/data-loader-and-preprocess.eps}
         \caption{Data pipeline in \SysName{} }.
         \label{figure:data_loader_preprocess_in_xFlow}
   %  \end{subfigure}
\end{figure}

As you can see, \SysName{} views everything as operators under actor design, and take the data loading and preprocess into the computing graph, to plan and schedule them optimally.

Two kinds of data precisions will be illustrated as follows.

1. Single precision(FP32) data movement in \SysName{}(see Figure \ref{figure:single_precision_data_movement})


\begin{figure}
     \centering
     %\begin{subfigure}[b]{0.12\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/oneflow_pipeline.eps}
         \caption{Single precision data movement in \SysName{}} 
         \label{figure:single_precision_data_movement} 
   %  \end{subfigure}

\end{figure}

In Figure \ref{figure:single_precision_data_movement}, Preprocessing and Training represent an executable graph consists of a group of ops(Transferred into Actors when it enters Runtime period) separately. Depend on the actor mechanism, a pipeline-parallel strategy will be employed as much as possible.
An \SysName{} data loading and preprocessing example in Runtime is illustrated in Figure \ref{figure:data_movement_example_oneflow}

\begin{figure}
     \centering
     %\begin{subfigure}[b]{0.12\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/time_line_oneflow.eps}
         \caption{Data movement example in \SysName{}}.
         \label{figure:data_movement_example_oneflow}
   %  \end{subfigure}
\end{figure}

As Figure \ref{figure:data_movement_example_OneFlow} shows, it describes a situation of overlapping data pre-procedure with computing. Different line styles separately represent data loading, data preprocessing, data transferring(CopyH2D) and training execute time in a batch. The white, grey, blue rectangles consist of 2 squares separately represent a pair of Registers which are free, busy, ready.
Generally, to label main time costs in training a model in descending order, it is training time of a batch, data preprocessing time, data loading time, CopyH2D time. Data has been always circulating in Registers with persistence, where the downward Register of data is busy being preprocessed once it has been fetched while the other Register is free that means it is ready for being loaded in section 1. In section 2, the downward Register is busy being delivered from the host to the device when the upward Register has done its own preprocessing which means it's free at this moment, but it will do training in no time. So does training downward Register and transferring upward Register. Noted that when CopyH2D time is short, the number of Registers of Preprocessing actor is 1 or 2 does not affect performance because data produced by the data preprocessing will be customed immediately, never occurring both 2 buffers occupied. Meanwhile, the number of CopyH2D Registers should be 2 to ensure Training could run immediately, not having to wait for data transferring.

In our tests, to decode picture data, even using all 24 cores which include 48 physical threads in the CPU, it could not meet the demand of training throughput of 10629 img/s with the 8 GPUs like V100 per node where we run ResNet50-v1.5. So we purpose a way of GPU decode via nvJPEG, which arrange image preprocessing work to GPU.

2. Auto Mixed Precisions(AMP) data movement in \SysName{}(see Figure \ref{figure:amp_data_movement})

\begin{figure}
     \centering
     %\begin{subfigure}[b]{0.12\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/oneflow_amp_data_movement.eps}
         \caption{AMP data movement in \SysName{} }.
         \label{figure:amp_data_movement}
   %  \end{subfigure}

\end{figure}

As Figure \ref{figure:amp_data_movement}  shows, Decode op reads images from host memory(CPU), and then decode images into device memory(GPU). Great ease to accomplish this case with actor mechanism in \SysName{}, where it only needs to add relevant modules in the forms of ops in the analysis graph. Afterward, on the one hand, it decodes images via GPU computing resource, on the other hand, it allocates practicable parallel strategy automatically from the system pipeline pool and applies it. In this way, it could settle with this bottleneck spontaneously.

Experimental comparisons between the other frameworks with DALI plug-in and \SysName{} with its original data loader are given as 
Fig \ref{figure:of_torch_tf_rn50} addresses the speed meliority of \SysName{} implementation even other frameworks plug DALI data loader and preprocess toolkit in.
For AMP experiments, results conveyed as follow,

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/of-torch-tf-rn50-fp32-com.eps}
         \caption{}.
         \label{figure:of_torch_tf_rn50}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/of-torch-tf-rn50-amp-com.eps}
         \caption{}.
         \label{figure:of_torch_tf_amp_rn50}
     \end{subfigure}
     \caption{Comparisons between the other frameworks with DALI plug-in and \SysName{} with its original data loader}
\end{figure}
 )

Figure \ref{figure:of_torch_tf_amp_rn50} interprets throughputs when applying AMP, which means it computers more quickly, so it aggravates throughputs if not to fetch data in time.

Implemented by actors in \SysName{}, it will apply every overlapping as it could to utilize every bit of computer power via just easily employing data loading into the logical graph, then actor mechanism will handle it naturally.

\subsection{Data-parallelism}

\jinhui{sunxue}
With bigger models and ever-increasing sizes of training datasets, distributed DNN systems take place to accelerate model training. When data computing could not catch up on the communication cost, resource waste occurs even though it uses multi-GPU, further as multi-node GPU clusters.

Data parallelism is commonly used in DNN training frameworks, such as Pytorch, TensorFlow, MXNet, and other frameworks[]. But
To specify that data is so important as the first citizen, we identify 3 key points in \SysName{} are summarized as follows:

1. Overlap the communication with computation as best it can: overlap the model synchronization(especially all reduce procedure) with backward propagation computation.

2. Less control overhead by using actor mechanism: Without a centralized schedule in the runtime, it will run faster.

3. Group all reduce operations into bigger adapted size: Gather the fragmented all reduce behaviors into a large one to cut communication times.

It's proof positive after having experiments in experiments. Based on those, we demonstrate that, after strictly aligning the configuration of existing frameworks and \SysName{}, \SysName{} outperforms the others for both fp32 and AMP (enabling dynamic loss scaling).

We typically picked popular models as ResNet50-v1.5 in CNN and BERT-base in NLP. For both models, we tested common batch size and maximum batch size and different precisions with the same configurations and the environment in the multi-GPU and multi-node cluster.

Major performance results of these two models(ResNet50-v1.5 and BERT) are summarized as Figure \ref{figure:rn50_b128_all}, \ref{figure:rn50_amp_256_all}, \ref{figure:bert_32_all}, \ref{figure:bert_max_all}:

\begin{comment}
\begin{figure}
     \centering
     \begin{minipage}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/rn50-b128-all.eps}
         \caption{FP32, batch size = 128}.
         \label{figure:rn50_b128_all}
     \end{minipage}
    \begin{minipage}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/rn50-amp-256-all.eps}
         \caption{AMP, batch size = 256}.
         \label{figure:rn50_amp_256_all}
    \end{minipage}
    \caption{ResNet5-v1.5 tests throughputs(images/sec)}.
\end{figure}   

\begin{figure}
        \begin{minipage}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/bert-32-all.eps}
    \caption{FP32, batch size =32}
         \label{figure:bert_32_all}
     \end{minipage}
        \begin{minipage}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/bert-max-all.eps}
         \caption{AMP, batch size = max}.
         \label{figure:bert_max_all}
     \end{minipage}
     \caption{BERT-base tests throughputs(sentences/sec)}.
\end{figure}
\end{comment}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/rn50-b128-all.eps}
         \caption{}.
         \label{figure:rn50_b128_all}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/rn50-amp-256-all.eps}
         \caption{}.
         \label{figure:rn50_amp_256_all}
     \end{subfigure}
     \caption{ResNet5-v1.5 tests throughputs(images/sec)}
\end{figure*}
 )

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/bert-32-all.eps}
         \caption{}.
         \label{figure:figure:bert_32_all}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/bert-max-all.eps}
         \caption{}.
         \label{figure:bert_max_all}
     \end{subfigure}
     \caption{BERT-base tests throughputs(sentences/sec)}
\end{figure*}
 )
 

%\end{comment}

\subsection{Model-Parallelism}
\subsubsection{Insightface}
\jinhui{sunxue}
Hybrid parallelism(data parallelism + model parallelism) achieves remarkable scores in solving the very large scale(magnitude order from billions to trillions) face recognition problem. But most frameworks do not provide an eminent design to combine the model with data parallelism flexibly like \SysName{}. For example, Insightface, an open-source 2D\&.3D deep face analysis toolbox, usually contains around the number of 80000-300000 faces, which makes the model too large to hold in one GPU card, so that it should use model parallelism after data-paralleled CNN feature extraction backbone. In MXNet, it uses more than 800-line codes to manually split the data into parts carefully and transfer them in a fixed route, in comparison, \SysName{} only needs no more than 10 lines in Python scripts, where just label the data route behaviors and then the actor and SBP will grab the relay baton in a breeze.

More than that, any loss type that supports model parallelism, where it means that it supports to split into the axis of the probabilities distribution in the feature map(or activation) tensor in the recognization tasks, could be seamlessly expanded via the programmable feature in the \SysName{} system. Otherwise, it has to add extra complicated computation and communication logic even reuse codes as much as possible.

Here are experiments' results on training the Insightface. It compared the throughputs between different training batch sizes in the \SysName{} and MXNet implementation separately with ResNet100 and Mobilefacenet as backbones and the same loss of Arcface(see Fig 1-4).
 
 \begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/of-mx-infc-r100-64.eps}
         \caption{Batch size = 64}.
         \label{figure:of_mx_r100_b64}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/of-mx-infc-r100-96.eps}
         \caption{Batch size = 96}.
         \label{figure:of_mx_r100_b96}
     \end{subfigure}
     \caption{ResNet100 as backbone to train Insightface}
\end{figure}

 \begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/of-mx-infc-r100-64.eps}
         \caption{Batch size = 128}.
         \label{figure:of_mx_r100_b64}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{figure/of-mx-infc-r100-96.eps}
         \caption{Batch size = 256}.
         \label{figure:of_mx_r100_b96}
     \end{subfigure}
     \caption{Mobilefacenet as backbone to train Insightface}
\end{figure}


\subsubsection{Wide and Deep}
\input{exp_wide_and_deep}

\subsubsection{Megatron-LM}
\input{exp_hybrid_parallel}

\subsection{Pipelining Parallelism and SSP}
\input{ssp}



\subsection{Optimizer Placement Optimization}
\input{exp_non-dist-opt}


==> discussions.tex <==
\vspace{-0.3cm}
\section{Discussions and Related Work}
%\vspace{-0.3cm}

%\noindent\textbf{DL frameworks and compilers.}

%\noindent\textbf{Enhancements.}

%Mesh-tensorflow
%Gpipe
%PipeDream

%InsightFace
%HugeCTR
%Megatron-LM
%DeepSpeed

%FlexFlow
%GShard
%TensorOpt

%Actor model is able to describe the deep learning runtime on a single device. Nevertheless, the actor model helps most in distributed deep learning. 

%infer the register number.

%why redesign

%\noindent\textbf{SBP configuration and auto-parallel.} The SBP configuration could be still too complex for the users to set. However, directly coding with communication primitives for a different kind of parallelism is more complicated. We transform the manually programming to setting \textit{SBP} signatures. Moreover, in \SysName{}, the user could just set the \textit{SBP} signatures of a subset of ops instead of the whole set, and leave the rest \textit{SBP} to be inferred with heuristic approach like GShard~\cite{dmitry-2020-gshard}, in which users provide some initial annotations or use default annotations as seed, then the algorithm propagates the sharding information to the un-annotated tensors. The approach in FlexFlow~\cite{jia-2019-sysml} can also be used here. 

%\paragraph{Whether the actor model is intrinsic?} Distributed deep learning is much more complicated than non-distributed one. The complexity of distributed deep learning originates from the dependency and resource management, such as avoiding OOM and deadlock, minimizing the stalls, etc. The design rationale of \SysName{} is that static planning of the resource is essential for efficient and stable distributed deep learning. Dynamic resource allocation will bring much more engineering efforts to achieve the same goal. The actor model provides a simple yet powerful runtime abstraction for the philosophy of static planning everything. The actor model solves the problem by adding a thin wrapper around the Ops, i.e., state management. The finite state machine in the actor model helps incorporate the resource constraint as part of the trigger condition. Actor model is able to describe the deep learning runtime on a single device. Nevertheless, the actor model helps most in distributed deep learning. In a single-device scenario, we might not gain apparent advantages over the traditional graph executor. This paper uses the actor model to unify the runtime of distributed training and non-distributed training.

\noindent\textbf{Actor model in Ray.} Even though both \SysName{} and Ray~\cite{phillipp-2017-ray} use the concept of the actor, the granularities are different. In Ray, a single actor is used to manage a complete neural network while performing deep learning training. So far, Ray can only act as a plugin to enable data-parallelism to Tensorflow and PyTorch. Besides the common data-parallelism, \SysName{} also supports model-parallelism and pipeline-parallelism. In \SysName{}, an actor is usually used to manage the state (dedicated resource and finite state machine) of a single operator/kernel and the interactions between operators (though in theory, it can also manage the state of a model). 

%\paragraph{Enable TensorFlow and PyTorch with the actor model} It is a great idea to push the actor's abstraction as a runtime layer underneath Pytorch or TensorFlow and show that the distributed training of Pytorch can benefit from the actor abstraction. We want to investigate such a possibility in the future. We notice that both TensorFlow and PyTorch teams are carrying out some relating efforts recently even they do not use the name of the actor model. For example, the core idea of two new projects initiated by PyTorch for distributed training, i.e., fairscale~\cite{fairscale} and tensorpipe~\cite{tensorpipe}, is message passing. The core idea of the new runtime project of Tensorflow~\cite{tensorflow-runtime} is an asynchronous runner similar to promise and future. The actor runtime system of \SysName{} is initiated four years ago.

%\paragraph{Why redesign the whole stack?} Redesigning a complicated system from scratch is not an easy decision. It involves many engineering efforts. A more natural choice is to build customized implementation on top of existing frameworks. Such examples include Nvidia Megatron-LM~\cite{mohanmmad-megatron-2020}, Microsoft PipeDream~\cite{narayanan-2019-sosp}, Microsoft DeepSpeed~\cite{rajbhandari-zero-2020}, Facebook FairScale~\cite{fairscale}, all of which are based on PyTorch, InsightFace~\cite{insightface} is based on MXNet. Nvidia even builds a library specialized for a recommendation system, i.e., HugeCTR~\cite{Oldridge2020MerlinAG}. We observe the emerging need for training deep learning models with an extremely large number of parameters, which brings novel challenges to the existing deep learning frameworks. Even though several efforts try to address the challenges by modifying or refining Tensorflow or PyTorch, we rethink the design of the deep learning framework by treating distributed training as the first principle. We propose that we need to redesign the distributed deep learning framework. \hz{doesn't really explained why we need a redesign.} We implement a deep learning framework \SysName{} with this design and show that the new design brings the advantages of simplicity and efficiency. The solution of \SysName{} is general enough to support all the ideas in the above customized system succinctly. In the evaluation, we compare \SysName{} with all the above customized implementation and observe the efficiency advantage.

\noindent\textbf{Parallel Strategies in Distributed Training.}
To support more complicated parallelism strategies, many schemes are proposed as wrappers or plugins based on some mainstream DL frameworks such as TensorFlow and PyTorch. Mesh-TensorFlow \cite{shazeer-2018-nips}, FlexFlow \cite{jia-2019-sysml} and GShard \cite{dmitry-2020-gshard} provide APIs for developers to express a wide range of parallel computation patterns for different components of DNN models. Among the existing work, GShard is most similar to the SBP abstraction proposed in this paper. The fundamental differences between the \textit{SBP} with the abstraction in GShard are discussed in Section \ref{sec:sbp}.
%\footnote{We develop \SysName{} with the SBP abstraction before we are aware of the Gshard paper. Just soon after Gshard is published, \SysName{} is open sourced at GitHub.}
Horovod~\cite{alexander-2018-horovod} achieves efficient data parallelism in a homogeneous environment with highly-optimized collective communication library NCCL \cite{jeaugey2017nccl}. Stanza \cite{wu2018stanza} and DLPlacer \cite{pal2019optimizing} adopt data parallelism for training convolutional layers in CNN models and model parallelism for other layers. OptCNN \cite{jia-2018-icml} parallelizes CNN model training by splitting operations along batch and channel dimensions on homogeneous devices. Tofu \cite{wang-2019-eurosys} utilizes a partition-n-reduce method to split a single operation into sub-operations and a dynamic programming approach to optimize the partition recursively; no device placement of operations is considered. FlexFlow \cite{jia-2019-sysml} explores the SOAP (sample, operation attribute, parameter) search space to address parallelism within and across operations. HeteroG \cite{yi2020optimizing}, Placeto \cite{addanki2018placeto} and GDP \cite{zhou2019gdp} utilize Graph Neural Network and reinforcement learning to produce efficient distributed strategies for various DNNs.

%Pipelining has been studied to accelerate DNN training: different DNN layers are deployed on different devices; a mini-batch is divided into micro-batches. The micro-batches can be processed at different devices concurrently.
GPipe \cite{huang-2019-nips} uses pipelining to address memory bottlenecks for training large DNNs. PipeDream \cite{narayanan-2019-sosp} introduces a pipelining approach to overlap communication and computation for asynchronous training. HetPipe \cite{hetpipe} integrates pipeline parallelism with data parallelism in a heterogeneous environment, making layer-based parallelism decisions. These pipelining strategies are all based on existing frameworks such as TensorFlow. Large amounts of sub-operations and control dependencies need to be added to the computation graph to achieve an efficient pipeline by DNN developers themselves. 

As we mentioned, most of these works are based on existing training frameworks that are not dedicated to such complicated parallelism strategies, which yields both great engineering efforts and non-negligible system overhead. 

%GPT-3~\cite{brown-gpt-2020}

%Scaling laws~\cite{kaplan-scaling-2020}

%swapadvisor~\cite{huang-swapadvisor-2020}

%aibox~\cite{zhao-aibox-2020}

%checkmate~\cite{jain-checkmate-2020}

==> exp_hybrid_parallel.tex <==
\xiexuan{}
To demonstrate \sys{}'s expandability to large language models, we consider training GPT models similar to Megatron-LM implementation. Benefit from SBP mechanism of \sys{}, \sys{} implements data, model hybrid parallelism simply and conveniently by setting SBP property of a tensor in GPT model. 

In \sys{} implementation, token embedding table is split by its vocabulary dimention(S(0)), after looking up operation with inputs as indices, every device gets only part of features, and then the features are reduce-scattered to all devices, data block shape is $D=[batch\_size, sequence\_length, hidden\_size]$, positional encoding vector is added in each device. before handing the features to the first layer of blocks, the features is broadcasted to all devices, data block shape is $D$. 

\sys{} applies the same intra-layer model-parallelism with Megatron-LM, the entrance fully-connected model is split by it's second dimension($SBP=S(1)$), and the exit fully-connected model is split by it's first dimension($SBP=S(0)$), 4 total all-reduce communication operations in the forward and backward pass of a single layer of block, data block shape of each all-reduce operation is $[batch\_size*sequence\_length, hidden\_size]$. 

GPT has a language model regression using matrix multiply operator to generate predition logits of each device with $SBP=S(1)$, following is the softmax cross entropy to calculate losses. In \sys{}, softmax cross entropy loss op accepts broadcasted labels and $S(1)$ split logits as inputs, and perform high efficiency and low cost computation and communication. 

Our test machine is a server with 8 Nvidia Tesla V100-16G GPUs, all tests are under auto mixed precision mode(FP16). To verify the performance of \sys{} GPT implementation, Megatron-LM GPT-2 model is tested in the same environment and with same configurations. The hidden size and the number of layer are varied to reach GPU memory limit but the hidden size per head is fixed to 96. The original vocabulary size is 50,257 and will be padded to 128*model parallel GPUs number. Total batch size is fixed to 8. Average latency of iteration and the max GPU memory usage were recorded.



\hanbinbin{}
Megatron-LM implements hybrid parallelism through precise analysis on transformer. It splits the weight matrix in different dimensions explicitly in transformer layers, which consists of a self attention block followed by a two-layer, multi-layer perceptron(MLP). Although it is very sample theoretically, it's not easy from the aspect of code and not generic enough, which needs in-depth analysis of model characteristics and insert code accurately into the model.

\hanbinbin{} TO test the performance of \sys{}, we train GPT-model based \sys{} and Nvidia Megatron-LM. This model uses data-parallelism and model-parallelism. Unlike Megatron, with \sys{}, we can implement data parallelism, model parallelism or any combination of them flexible and convenient. Based on SBP mechanism, What we need is only simply configuring the correct information information of workers and setting the SBP property of a tensor. Then \sys{} will insert boxing nodes automatically and generete the corresponding physical execution diagram you want, which is very convenient and low cost for you.

\jinhui{xiexuan, xiexuan} \hanbinbin{del this paragraph} By training GPT-model, we compare \sys{} and Nvidia Megatron-LM. This model uses data-parallelism, model-parallelism and pipelining-parallelism \hanbinbin{no pipelining-parallelism here}. The result show that \sys{} is much faster than Nvidia Megatron-LM.

\xiexuan{}
GPT model has three major parts, input embedding, stack of decoder blocks and language model regression module. Input embedding includes token embedding and position embedding. Every decoder block has two layers: a masked self-attention layer and a feed forward layer(mlp), both attention layer and mlp layer have two fully-connected operators placed at the entrance and exit of the layer respectively. Output features is multiplied by token embedding, which produces the prediction of token logits(probabilities).

In GPT series models, embedding size(hidden size) and number of decoder blocks are two major hyper-parameters which impact GPT model size, plus context size(sequence length), the three of them determine the size of activations.

In \sys{} implementation, token embedding table is splited by its vocabulary dimention(S(0)), after looking up operation with inputs as indices, every device gets only part of features, and then the features are reduce-scattered to all devices, data block shape is $D=[batch\_size, sequence\_length, hidden\_size]$, positional encoding vector is added in each device. before handing the features to the first layer of blocks, the features is broadcasted to all devices, data block shape is $D$. 

\sys{} applies the same intra-layer model-parallelism with Megatron-LM, the entrance fully-connected model is split by it's second dimension($SBP=S(1)$), and the exit fully-connected model is split by it's first dimension($SBP=S(0)$), 4 total all-reduce communication operations in the forward and backward pass of a single layer of block, data block shape of each all-reduce operation is $[batch\_size*sequence\_length, hidden\_size]$. 

GPT has a language model regression using matrix multiply operator to generate predition logits of each device with $SBP=S(1)$, following is the softmax cross entropy to calculate losses. In this part \sys{} uses the same model parallel strategy in 7.4.1    Insightface.

Test node is a server with 8 V100-16G GPUs, all tests are under auto mixed precision mode(FP16). To verify the performance of \sys{} GPT implementation, Megatron-LM GPT-2 model is considered as the reference. The hidden size and the number of layer are varied to reach GPU memory limit. The original vocabulary size is 50,257 and will be padded to 128*model parallel GPUs number. Total batch size is fixed to 8 and hidden size per head is fixed to 96. Latency per iteration and the max GPU memory usage were recorded and reported.

\begin{table*}
    \centering
    \begin{tabular}{|p{1.2cm}<{\centering}|p{1.2cm}<{\centering}|p{1.2cm}<{\centering}|p{1.2cm}<{\centering}|c|c|c|c|}
    \hline
    \multirow{3}{*}{\makecell[c]{Hidden \\ Size}} 
    & \multirow{3}{*}{\makecell[c]{Attention \\ heads}} 
    & \multirow{3}{*}{\makecell[c]{Number \\ of \\ Layers}}
    & \multirow{3}{*}{\makecell[c]{ Model \\ Parallel \\ GPUs }}
    & \multicolumn{2}{c|} { Megatron-LM }
    & \multicolumn{2}{c|} { \sys{} } \\
    \cline{5-8} & & & & Memory & Latency & Memory & Latency \\ 
    & & & & (MiB) & (ms) & (MiB) & (ms)\\
    \hline
        1536 & 16 & 14 & 1 & 14947 & 768.4 & 12689 & 715.7 \\ \hline
        1920 & 20 & 20 & 2 & 15635 & 957.9 & 15597 & 860.6 \\ \hline
        2304 & 24 & 22 & 4 & 13813 & 725.7 & 15217 & 707.8 \\ \hline
        2688 & 32 & 24 & 8 & 11745 & 702.9 & 15535 & 690.4 \\ \hline
    \end{tabular}
    \caption{GTP Model Parallel Test Result}
    \label{tab:GTP-MODLE}
\end{table*}

Table \ref{tab:GTP-MODLE} shows \sys{} runs faster than Megatron-LM, Megatron-LM consumes less GPU memory than \sys{}, \sys{} will update memory management strategy by adding dynamic memory pool for NCCL thread which will reduce memory consumption. 



==> exp_non-dist-opt.tex <==
%backup 2021.5.7

\subsection{Parallelizing the Optimizer}
%\vspace{-0.3cm}
For large model training, model states (such as gradients, parameters, momentum and variances in Adam) related with optimizer occupy the majority of the memory. Data parallelism replicates the entire model states across all devices which is not necessary. Each device can update one part of model states and get the full parameter with AllGather. With this approach, data parallelism enables much larger model size. Deep-Speed project implements this idea as \emph{ZeRO}-DP \cite{rajbhandari-2020-zero}. \SysName{} provides a similar implementation which we refer to as %named
\emph{Optimizer-Placement-Optimization}. As shown in Figure~\ref{figure:zero}, %to implement this optimization in \sys{},
the main change with this optimization in \sys{} is to modify the SBP annotations of the optimizer states \cwu{what optimizer states are, are not discussed in the paper } from Broadcast to Split in the logical graph \cwu{give the rationale why this leads to some optimization}. The physical tensor operations and communication operations are then %all 
generated  automatically. \jinhui{explain more} Such implementation in \sys{} is far more simple and clean than %Deep-Speed's
\emph{ZeRO}-DP. Figure \ref{figure:deep_speed} compares per-device memory footprint %reduction
and throughput when training GPT-2 with and without this optimization, with the activation checkpoint off \cwu{what does `with the activation checkpoint off' mean}. \cwu{explain what the ..theoretical.. cases are} We can conclude that the more devices we use, the more memory footprint reduction %on models states we will get. 
we obtain. \cwu{how do you observe the reduction, comparing which case to which case? Briefly comment on the throughput comparison as well.}



% 2021.5.7

\jinhui{luyang, xiaoyu, depeng}The memory redundancy of model states in data-parallel can be reduced by splitting them across devices. Each device only needs to compute a part of the parameters and use an all-gather operation to get the whole parameters. Recently, Microsoft released Deep-Speed\footnote{https://github.com/microsoft/deepspeed} \emph{ZeRO}-DP \cite{rajbhandari2020zero} to realize this idea. We have also implemented the similar optimization in \sys{} named \emph{Optimizer-Placement-Optimization}.


Let's take Adam\cite{kingma2017adam} optimizer and mixed precision training as a concrete example. Assume the model has $\Psi$ parameters and the number of devices is $N$. For mixed precision data-parallel training, \sys{}'s \emph{Optimizer-Placement-Optimization} uses static memory allocation strategy, the memory footprint will reduce from $22\Psi$ bytes to \((4 + \frac{20}{N})\Psi\) bytes. And \emph{ZeRO}-DP uses dynamic memory allocation strategy and the memory footprint will reduce from $16\Psi$ bytes to \((4 + \frac{12}{N})\Psi\) bytes. Table \ref{tab:non-dist-opt} and Table \ref{tab:zero-dp} shows the theoretical and measured memory footprint reduction with this optimization. In these tables, \#S, \#G and \#B denote the number of servers, GPUs on each server and batch-size on each GPU respectively. The units of per-device throughput is $samples/second$. We can conclude that the more devices we used the more memory footprint reduction on models states we will get.


\emph{ZeRO}-DP's implementation was based on PyTorch's Tensor operations and Distributed Communication Package, which takes about 2000 lines of codes. On contrast, our implementation named \emph{Optimizer-Placement-Optimization} is just a rewriting pass of forward logical graph to adjust the SBP signature, which only takes about 300 lines of codes.

\emph{Optimizer-Placement-Optimization} has three main steps. Firstly, for every parameter on the logical graph, link its successor converting operations(such as \textit{fp}16 cast) as a parameter converting chain. Secondly, for each chain, modify the SBP signature of the first node to $split$ and the successors of the last node to $broadcast$, which is depicted in Figure \ref{figure:non_dis_overivew1}. Thirdly, insert control edges between these chains according to the topological order of each chain's successors. In this way, the earlier the parameter is used, the corresponding all-gather opeartion is conducted earlier to generate the complete parameter.

During the physical graph compilation phase, the corresponding backward and model update computation graphs will be generated automatically. The generated backward and model update computation graphs are depicted in Figure \ref{figure:non_dis_overivew2}.

As we can see, to implement this optimization, the main thing we need to do is changing the SBP signature of parameters on the forward logical computation graph. The physical tensor operations and communication operations are all generated  automatically for the full training process. This makes our implementation in \sys{} far more simple and clean than Microsoft Deep-Speed's \emph{ZeRO}-DP which is based on Tensor Operations and Collection Communication operations.


% \usepackage{multirow}
\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
    \hline
    \multirow{2}{*} {Model \& Size(MB) } & \multirow{2}{*} {\#S$\times$\#G$\times$\#B}
    & \multicolumn{2}{c|} {Optimization Off} & \multicolumn{2}{c|} {Optimization On}
    & \multicolumn{2}{c|} {\textbf{Memory reduction}(MB)} \\
    \cline{3-8}
      & & Memory & Throughput & Memory & Throughput  & \textbf{Theoretical} & \textbf{Measured} \\ 
    \hline
    GPT-2-small, 474 & 1$\times$4$\times$4 & 11209 & 29.8 & 9881 & 29.3 & 1543 & 1328 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$4 & 11500 & 28.8 & 9755 & 27.9 & 1840 & 1745 \\
    \hline
    GPT2-small, 474 & 2$\times$8$\times$4 & 11087 & 25.8 & 9160 & 24.7 & 1988 & 1927 \\
    \hline
    GPT2-small, 474 & 4$\times$8$\times$4 & 11089 & 22.4 & 9082 & 23.2 & 2062 & 2007 \\
    \hline
    \end{tabular}
    \caption{Per-device memory reduction and per-device throughput of \sys{}'s \emph{Optimizer-Placement-Optimization}. The measured memory reduction matches the theoretical value which demonstrates our memory analysis provides the realistic estimation.}
    \label{tab:non-dist-opt}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|} 
    \hline
    \multirow{2}{*} {Model \& Size(MB) } & \multirow{2}{*} {\#S$\times$\#G$\times$\#B}
    & \multicolumn{2}{c|} {Optimization Off} & \multicolumn{2}{c|} {Optimization On}
    & \multicolumn{2}{c|} {\textbf{Memory reduction}(MB)} \\
    \cline{3-8}
      & & Memory & Throughput & Memory & Throughput  & \textbf{Theoretical} & \textbf{Measured} \\ 
    \hline
    GPT-2-small, 474 & 1$\times$4$\times$4 & 15363 & 24.8 & 14331 & 24.8 & 1068 & 1032 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$4 & 15387 & 24.9 & 14199 & 24.5 & 1246 & 1188 \\
    \hline
    GPT-2-small, 474 & 2$\times$8$\times$4 & 15336 & 16.8 & 14005 & 16.3 & 1335 & 1331 \\
    \hline
    GPT-2-small, 474 & 4$\times$8$\times$4 & 15336 & 16.7 & 13975 & 15.8 & 1380 & 1361 \\
    \hline
    \end{tabular}
    \caption{Per-device memory reduction and per-device throughput of \emph{ZeRO}-DP's Optimizer State Partitioning \cite{rajbhandari2020zero}}.
    \label{tab:zero-dp}
\end{table*}



\begin{figure*}[ht]
       \centering
          \includegraphics[width=\textwidth]{figure/non_dis_overview_1.png}
          \caption{Demonstrates the \emph{Optimizer-Placement-Optimization} process on 2 GPUs in \sys{}. The boxing nodes are inserted automatically during the graph compilation phase.}
         \label{figure:non_dis_overivew1}
\end{figure*}

\begin{figure*}[ht]
       \centering
          \includegraphics[width=\textwidth]{figure/non_dis_overview_2.png}
          \caption{Demonstrates auto-generated backward and model update graph of the \emph{Optimizer-Placement-Optimization} on 2 GPUs in \sys{}. Also the boxing nodes are inserted automatically during the graph compilation phase.}
         \label{figure:non_dis_overivew2}
\end{figure*}







\begin{comment}

we conducted the experiments on a cluster of 16 V100 GPUs ( 2 DGX-1 nodes ?) with 100 Gbps internode communication bandwidth.


backup compressed version:

The memory redundancy of model states in data-parallel can be reduced by splitting them across devices. Each device only needs to hold a part of the parameters and use an all-gather operation to get the complete parameters before forward propagation. Recently, Microsoft released Deep-Speed\footnote{https://github.com/microsoft/deepspeed} \emph{ZeRO}-DP \cite{rajbhandari2020zero} to realize this idea. We have also implemented the similar optimization in \sys{} named \emph{Optimizer-Placement-Optimization}.


Let's take Adam\cite{kingma2017adam} optimizer and mixed precision training as a concrete example. Assume the model has $\Psi$ parameters and the number of devices is $N$. For mixed precision data-parallel training, \sys{}'s \emph{Optimizer-Placement-Optimization} uses static memory allocation strategy, the memory footprint will reduce from $22\Psi$ bytes to \((4 + \frac{20}{N})\Psi\) bytes. And \emph{ZeRO}-DP uses dynamic memory allocation strategy and the memory footprint will reduce from $16\Psi$ bytes to \((4 + \frac{12}{N})\Psi\) bytes. Figure \ref{fig:deep_speed} shows per-device memory footprint reduction and throughtput with this optimization. We can conclude that the more devices we used the more memory footprint reduction on models states we will get.


\emph{ZeRO}-DP's implementation was based on PyTorch's Tensor operations and Distributed Communication Package, which takes about 2000 lines of codes. On contrast, our implementation named \emph{Optimizer-Placement-Optimization} is just a rewriting pass of forward logical graph to adjust the SBP signature, which only takes about 300 lines of codes.

\emph{Optimizer-Placement-Optimization} has three main steps. Firstly, for every parameter on the logical graph, link its successor converting operations(such as \textit{fp}16 cast) as a parameter converting chain. Secondly, for each chain, modify the SBP signature of the first node to $split$ and the successors of the last node to $broadcast$. Thirdly, insert control edges between these chains according to the topological order of each chain's successors. In this way, the earlier the parameter is used, the corresponding all-gather opeartion is conducted earlier to generate the complete parameter.

During the physical graph compilation phase, the corresponding backward and model update computation graphs will be generated automatically. 

As we can see, to implement this optimization, the main thing we need to do is changing the SBP signature of parameters on the forward logical computation graph. The physical tensor operations and communication operations are all generated  automatically for the full training process. This makes our implementation in \sys{} far more simple and clean than Microsoft Deep-Speed's \emph{ZeRO}-DP which is based on Tensor Operations and Collection Communication operations.



backup full version:
\jinhui{luyang, xiaoyu, depeng}For training large models, the majority of the device memory is occupied by the activations and model states including parameters, gradients and optimizer states (such as momentum and variances in Adam \cite{kingma2017adam}). Basic data-parallelism implementation will replicates the entire model states across all devices which results in redundant memory consumption. Recently, Microsoft released Deep-Speed\footnote{https://github.com/microsoft/deepspeed} to optimize the memory redundance of data parallelism which is called \emph{ZeRO}-DP \cite{rajbhandari2020zero}. Prior to the debut of Deep-Speed, we independently found the optimization opportunity and turned our idea into an implementation in \sys{} named \emph{Optimizer-Placement-Optimization}.

\chengcheng{ This section of \emph{Optimizer-Placement-Optimization} is too long, which took 2 pages. In the end, it should be compressed to less than 1 page. We don't need to explain in detail how ZeRO does it, just cite their paper directly. Specifically, readers can read ZeRO paper. But don’t delete it first, you can use comment them out and then extract short content. }

The redundancy of model states in data-parallel can be optimized by splitting them across devices. By doing so, each device only need to allocate and compute a part of the model states. Let's take Adam optimizer and mixed precision training as a concrete example. When training a model with $\Psi$ parameters using data parallel, each device needs to hold the entire \textit{fp}16 gradients ($2\Psi$ bytes). After the backward propagation, an all-reduce operation is conducted on the \textit{fp}16 gradients ($2\Psi$ bytes). Then the \textit{fp}16 gradients will be cast to \textit{fp}32 ($4\Psi$ bytes) and used to compute the \textit{fp}32 momentum ($4\Psi$ bytes) and variance ($4\Psi$ bytes). At last, use these states to update the \textit{fp}32 parameters ($4\Psi$ bytes) which will be cast to \textit{fp}16 ($2\Psi$ bytes) for the next forward propagation. \sys{} uses static memory allocation strategy and the memory requirements for model states on each device is $22\Psi$ bytes.\chengcheng{ It is best to add some variable names to this part, and then 'total model states = a + b + c + d ... = $22\Psi$' }  On contrast,  \emph{ZeRO}-DP baseline uses dynamic memory allocation strategy and the memory requirements on each deivce is $16\Psi$ bytes. Let $N$ denotes the number of devices in data parallel, if we split the \textit{fp}16 gradients ($2\Psi$ bytes) equally across devices, then after the backward propagation, a reduce-scatter operation will be conducted to get the sliced \textit{fp}16 gradients (\(\frac{2\Psi} {N}\) bytes), which means we only needs \(\frac{1} {N}\) memory to compute the \(\frac{1} {N}\) partition  of parameters on each device. At last, an all-gather operation will be conducted to get the entire new \textit{fp}16 parameters ($2\Psi$ bytes) on each device.

% \usepackage{multirow}
\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
    \hline
    \multirow{2}{*} {Model \& Size(MB) } & \multirow{2}{*} {\#S$\times$\#G$\times$\#B}
    & \multicolumn{2}{c|} {Optimization Off} & \multicolumn{2}{c|} {Optimization On}
    & \multicolumn{2}{c|} {\textbf{Memory reduction}(MB)} \\
    \cline{3-8}
      & & Memory & Throughput & Memory & Throughput  & \textbf{Theoretical} & \textbf{Measured} \\ 
    \hline
    GPT-2-small, 474 & 1$\times$4$\times$4 & 11209 & 29.8 & 9881 & 29.3 & 1543 & 1328 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$4 & 11500 & 28.8 & 9755 & 27.9 & 1840 & 1745 \\
    \hline
    GPT2-small, 474 & 2$\times$8$\times$4 & 11087 & 25.8 & 9160 & 24.7 & 1988 & 1927 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$1 & 5655 & 12.5 & 3901 & 10.3 & 1840 & 1754 \\
    \hline
    GPT-2-medium, 1354 & 1$\times$8$\times$1 & 11969 & 6 & 7460 & 5.1 & 5256 & 4509 \\
    \hline
    \end{tabular}
    \caption{Per-device memory reduction and per-device throughput of \sys{}'s \emph{Optimizer-Placement-Optimization}. The measured memory reduction matches the theoretical value which demonstrates our memory analysis provides the realistic estimation.}
    \label{tab:non-dist-opt}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|} 
    \hline
    \multirow{2}{*} {Model \& Size(MB) } & \multirow{2}{*} {\#S$\times$\#G$\times$\#B}
    & \multicolumn{2}{c|} {Optimization Off} & \multicolumn{2}{l|} {Optimization On}
    & \multicolumn{2}{c|} {\textbf{Memory reduction}(MB)} \\
    \cline{3-8}
      & & Memory & Throughput & Memory & Throughput  & \textbf{Theoretical} & \textbf{Measured} \\ 
    \hline
    GPT-2-small, 474 & 1$\times$4$\times$4 & 15363 & 24.8 & 14331 & 24.8 & 1068 & 1032 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$4 & 15387 & 24.9 & 14199 & 24.5 & 1246 & 1188 \\
    \hline
    GPT-2-small, 474 & 2$\times$8$\times$4 & 15336 & 16.8 & 14005 & 16.3 & 1335 & 1331 \\
    \hline
    GPT-2-small, 474 & 1$\times$8$\times$1 & 6591 & 12.8 & 4945 & 12.3 & 1246 & 1646 \\
    \hline
    GPT-2-medium, 1354 & 1$\times$8$\times$1 & 14945 & 6.1 & 10799 & 6.4 & 3559 & 4146 \\
    \hline
    \end{tabular}
    \caption{Per-device memory reduction and per-device throughput of \emph{ZeRO}-DP's Optimizer State Partitioning \cite{rajbhandari2020zero}}.
    \label{tab:zero-dp}
\end{table*}

Microsoft Deep-Speed's \emph{ZeRO}-DP implements this idea which reduces memory footprint from $16\Psi$ bytes to \((4 + \frac{12}{N})\Psi\) bytes. \sys{} \emph{Optimizer-Placement-Optimization} also implements the same idea with the memory footprint reduction from $22\Psi$ bytes to \((4 + \frac{20}{N})\Psi\) bytes. In addition, a reduce-scatter operation combined with an all-gather operation in this optimization has the same communication volume as an all-reduce operation in the baseline implementation. So this idea eliminates memory redundancies in data-parallel training while retaining low communication volume. Table \ref{tab:non-dist-opt} and Table \ref{tab:zero-dp} shows the theoretical and measured memory footprint reduction with this optimization. In these tables, \#S, \#G and \#B denote the number of servers, GPUs on each server and batch-size on each GPU respectively. The units of per-device throughput is $samples/second$. We can conclude that the more devices we used the more memory footprint reduction on models states we will get. 


\begin{figure*}[ht]
       \centering
          \includegraphics[width=\textwidth]{figure/optimizer_placement_forward.eps}
          \caption{Demonstrates the \emph{Optimizer-Placement-Optimization} process on 2 GPUs in \sys{}. The boxing nodes are inserted automatically during the graph compilation phase.}
         \label{figure:non_dis_overivew1}
\end{figure*}

\begin{figure*}[ht]
       \centering
          \includegraphics[width=\textwidth]{figure/non_dis_overview_2.png}
          \caption{Demonstrates auto-generated backward and model update graph of the \emph{Optimizer-Placement-Optimization} on 2 GPUs in \sys{}. Also the boxing nodes are inserted automatically during the graph compilation phase.}
         \label{figure:non_dis_overivew2}
\end{figure*}

Both Microsoft Deep-Speed's \emph{ZeRO}-DP and our \emph{Optimizer-Placement-Optimization} can achieve the same goal but with very different implementation costs. We will see that programming on \sys{}'s actor system is much easier than programming with Tensor Operations or Collection Communication operations.

\textbf{\emph{ZeRO}-DP}'s implementation was based on PyTorch's Tensor operations and Distributed Communication Package. To control the backward stage of training process, \emph{ZeRO}-DP inherits the nn.Module and overrides the backward function. In the customized backward function, gradients tensor are partitioned and reduce-scattered by hand. To control the model update stage, an optimizer wrapper was created. In the optimizer wrapper, gradient partitions are created and the original optimizer was call to compute the new parameters sub partitions, then an all-gather operation was call to get the full parameters. Programming on basis of Tensor Operations or Collection Communication operations needs to carefully deal with all the data operation and communication by hand. To realize the model states optimization, about 2000 lines of code are crafted.


\textbf{Optimizer-Placement-Optimization} implements the model states memory footprint reduction by adjusting the SBP signature of the data-parallel operations' parameter in the forward computation graph, which has three main steps. Firstly, for every parameter $P$ on the graph, if its successor operation namely $O$ has only one input and output, then $P$ and $O$ will be linked as a chain. And then check the successor operation of $O$ to see whether it can be added to the chain. Continue this process until finding a successor that unsatisfied the constraint then put this chain into the chain group. Secondly, for each chain, modify the SBP signature of the first node to split and the successors of the last node to broadcast, which is depicted in Figure \ref{figure:non_dis_overivew1}.\chengcheng{ The following figure is a physical picture and will be more complicated. There should be a figure of the rewriting of the logic graph first. A pass which simply modify the Placement and insert an parallel cast op can do all thing in ZeRO. The boxing in the physical graph below is that our SBP and compile time automatically complete. } Thirdly, sort the chain group incrementally by the minimum topological order of each chain's successor. And then insert control edges between these chains in order to make sure the all-gather operations are also triggered in topological order, which can hopefully overlap the communication with computation better.

The SBP signature adjustment in \sys{} is just a pass of forward logical graph reweriting which only takes about 300 lines of codes. During the graph compilation phase, the corresponding backward and model update computation graphs will be generated automatically, the reduce-scatter operations will be inserted in the model update computation graph to get part of the full gradients automatically, an all-gather operation will also be inserted between the last node of each chain and its successors to get full updated parameters on each device automatically. The generated backward and model update computation graphs are depicted in Figure \ref{figure:non_dis_overivew2}.

As we can see, to implement this optimization, the main thing we need to do is changing the SBP signature of parameters on the forward logical computation graph. The physical tensor operations and communications are all generated for the full training process automatically. This makes our implementation in \sys{} far more simple and clean than Microsoft Deep-Speed's \emph{ZeRO}-DP which is based on Tensor Operations and Collection Communication operations.

To further reduce the memory footprint of data-parallel in \sys{}, the entire \textit{fp}16 gradients ($2\Psi$ bytes) and parameters ($2\Psi$ bytes) can be released immediately after use by introducing dynamic memory allocation strategy and result re-computation\cite{chen2016training} in the near future, which can also be implemented as configurable computation graph compile strategies in our system.


\end{comment}

==> exp_wide_and_deep.tex <==
% mainly solved problem and strategy
Wide \& Deep Leaning \cite{cheng2016wide} is widely used in recommender systems for Click-Through Rates estimation. It combines two sub models,
Wide model and Deep model with a
embedding matrix in each of them.
In production,
to support Click-Through Rates estimation system for billions of IDs,
the two embedding matrices are too large for a single GPU.
What's more, the cost to synchronize gradients in back propagation grows with the size of the embedding.
Thus,
for a large Wide \& Deep model,
model-paralleled on embedding table is absolutely necessary.

% compare the performance of hugectr and oneflow
When training Wide \& Deep model with model-parallel,
\sys{} outperforms HugeCTR in NVIDIA Merlin \cite{Oldridge2020MerlinAG},
a dedicated framework for training Click-Through Rates estimation model.
In our evaluation on Wide \& Deep training task, as shown in Figure \ref{figure:hugectr_of_latency_memory}, \sys{} has lower latency and less memory footprint compared to HugeCTR. As a result, \sys{} can train larger on Wide \& Deep model with the same hardware resources.


% implementation
HugeCTR\footnote{https://github.com/NVIDIA/HugeCTR} is written in CUDA C++ and highly exploits GPU-accelerated libraries such as cuBLAS, cuDNN, and NCCL. To enable efficient model-parallel on embedding layer, HugeCTR implements more than 20 customized operations such as $init$, $forward$, $backward$, $update\_params$, $all\_gather$, $sync\_all\_gpus$, etc. To outperform TensorFlow, HugeCTR build a highly customized system on bare ground for recommender model training.

In contrast, \sys{} is a generic framework for all kinds of deep learning tasks. Training Wide \& Deep on \sys{} with model parallelism doesn't required any extra domain-specific modifications to the core system, which can perfectly reuses other highly-optimized components including data loading,
post-processing and transparent distributed training.

To be more specific, in \sys{}'s implementation, users only need to set the SBP signature of the embedding table manually. Then the collective communication primitives for model parallelism will be inferred automatically.

In this case, the reduce-scatter and all2all operations are  automatically inserted into the physical coimputation graph of Wide \& Deep model respectively. While in HugeCTR every type of collective communication operation is added in the model in an ad hoc way.

Besides, training Wide \& Deep in \sys{} can also take advantage of the built-in optimizations to boost the performance, which include the computation and communication overlap and the memory reuse optimization.



\begin{comment}

The compressed version:

Wide \& Deep Leaning \cite{cheng2016wide} is widely used in recommender systems for Click-Through Rates estimation. It combines two sub models,
Wide model and Deep model with a
embedding matrix in each of them.
In production,
to support Click-Through Rates estimation system for billions of IDs,
the two embedding matrices are too large for a single GPU.
What's more, the cost to synchronize gradients in back propagation grows with the size of the embedding.
Thus,
for a large Wide \& Deep model,
model-paralleled on embedding table is absolutely necessary.

% compare the performance of hugectr and oneflow
When training Wide \& Deep model with model-parallel,
\sys{} outperforms HugeCTR in NVIDIA Merlin \cite{Oldridge2020MerlinAG},
a dedicated framework for training Click-Through Rates estimation model.
In our evaluation on Wide \& Deep training task, as shown in Figure \ref{figure:hugectr_of_latency_memory}, \sys{} has lower latency and less memory footprint compared to HugeCTR. As a result, \sys{} can train larger on Wide \& Deep model with the same hardware resources.


HugeCTR\footnote{https://github.com/NVIDIA/HugeCTR} is written in CUDA C++ and highly exploits GPU-accelerated libraries such as cuBLAS, cuDNN, and NCCL. To enable efficient model-parallel on embedding layer, HugeCTR implements more than 20 customized operations such as $init$, $forward$, $backward$, $update\_params$, $all\_gather$, $sync\_all\_gpus$, etc. To outperform TensorFlow, HugeCTR build a highly customized system on bare ground for recommender model training. In contrast, \sys{} is a generic framework for all kinds of deep learning tasks. Training Wide \& Deep on \sys{} with model parallelism doesn't required any extra domain-specific modifications to the core system, which can perfectly reuses other highly-optimized components including data loading, post-processing and transparent distributed training.

To be more specific, in \sys{}'s implementation, users only need to set the SBP signature of the embedding table manually. Then the collective communication primitives for model parallelism will be inferred automatically. In this case, the reduce-scatter and all2all operations are  automatically inserted into the physical coimputation graph of Wide \& Deep model respectively. While in HugeCTR every type of collective communication operation is added in the model in an ad hoc way. Besides, training Wide \& Deep in \sys{} can also take advantage of the built-in optimizations to boost the performance, which include the computation and communication overlap and the memory reuse optimization.


\end{comment}


==> interface.tex <==
\vspace{-0.3cm}
\subsection{The Programming Interface}\label{sec:api}
\vspace{-0.2cm}

%\begin{table}[]
%\begin{tabular} {c}
%\hline 

%\begin{lstlisting}[language=Python]
%import xflow as xf
%P = xf.placement("cuda", {0:[0,1]})
%x_sbp = xf.sbp.split(0)
%w_sbp = xf.sbp.broadcast
%x = xf.randn(4,5,placement=P, sbp=x_sbp)
%w = xf.randn(5,8,placement=P, sbp=w_sbp)
%y = xf.matmul(x,w)    
%\end{lstlisting}\\

%\hline 
%\end{tabular}
%\caption{Data parallelism of a matrix multiplication operator.}
%\label{tab:data_parallelism}

%\end{table}

%\begin{table}[]
%\begin{tabular} {c}
%\hline 

%\begin{lstlisting}[language=Python]
%import xflow as xf
%P = xf.placement("cuda", {0:[0,1]})
%x_sbp = xf.sbp.broadcast
%w_sbp = xf.sbp.split(1)
%x = xf.randn(4,5,placement=P, sbp=x_sbp)
%w = xf.randn(5,8,placement=P, sbp=w_sbp)
%y = xf.matmul(x,w)      
%\end{lstlisting}\\

%\hline 
%\end{tabular}
%\caption{Model parallelism of a matrix multiplication operator.}
%\label{tab:model_parallelism}

%\end{table}

\begin{table}[]
\begin{tabular} {c}
\hline 

\begin{lstlisting}[language=Python]
import oneflow as flow
P0 = flow.placement("cuda", {0:[0,1]})
P1 = flow.placement("cuda", {1:[0,1]})
a0_sbp = flow.sbp.split(0)
b0_sbp = flow.sbp.broadcast
y0_sbp = flow.sbp.broadcast
b1_sbp = flow.sbp.split(1)

A0 = flow.randn(4,5,placement=P0,sbp=a0_sbp)
B0 = flow.randn(5,8,placement=P0,sbp=b0_sbp)
Y0 = flow.matmul(A0,B0) 

Y0.to_consistent(placement=P1,sbp=y0_sbp)
B1 = flow.randn(8,6,placement=P1,sbp=b1_sbp)
Y2 = flow.matmul(Y0,B1)
\end{lstlisting}\\

\hline 
\end{tabular}
\caption{Data parallelism for the first matmul Op, model parallelism for the second matmul Op, the two matmul Ops work with pipeline parallelism.}
\label{tab:api_demo}
\end{table}

Take the case illustrated in Figure \ref{figure:sbp_translation} as an example, the $MatMul_{0}$ suits to data-parallelism while the $MatMul_{1}$ suits to model-parallelism. The code snippet in Table \ref{tab:api_demo} illustrates how \SysName{} supports data-parallelism for $MatMul_{0}$ and model-parallelism for $MatMul_{1}$. Line 2 and line 3 introduce two different placements, the string \textit{cuda} indicates the type of accelerator is NVIDIA GPGPU, the structures $\{0:[0,1]\}$ and $\{1:[0,1]\}$ indicate the concrete location of the devices, i.e., the number before the colon is the node ID and the numbers in square bracket are the devices IDs. Note that $P0$ and $P1$ are different, they locate on node 0 and node 1 respectively. The variables from line 4 to line 7 represent several \textit{SBP} signatures. In \SysName{}, the placement and \textit{SBP} attributes of each tensor is either explicitly specified by developers (e.g., lines 9, 10, 14) or implicitly inferred by \SysName{} (e.g., in line 11, the \textit{SBP} of $Y_{0}$ can be inferred as $split(0)$). %In this way, the interface of operators remains unchanged no matter in non-distributed or in distributed scenarios, while other frameworks usually need to decorate the operators and the model description in order to support distributed training. 
In line 13, \SysName{} uses \emph{to\_consistent()} method to explicitly transform the placement and \textit{SBP} signature of a tensor. Note that, since the placements of the input tensors for $MatMul_{0}$ and $MatMul_{1}$ are different, i.e., $P0$ and $P1$ respectively, the two operators actually work with pipeline parallelism.

\SysName{} does not require the users to directly program with the various low-level communication primitives, users still need to think of the appropriate placement and \textit{SBP} signatures for each tensor. Manually specifying placement and \textit{SBP} signatures seems to be still too complex for the developers. Before completely solving the auto-placement and auto-parallelism challenges, a few techniques can be used to reduce the mental burden. For example, the user could just set the \textit{SBP} signatures of a subset of tensors instead of the whole set, and leave the rest \textit{SBP} to be inferred with heuristic approach like GShard~\cite{dmitry-2020-gshard}, in which users provide some initial annotations or use default annotations as seed, then the algorithm propagates the sharding information to the un-annotated tensors. The approach in FlexFlow~\cite{jia-2019-sysml} can also be used here.

%The above programming interface helps the users develop distributed deep learning models just like on a single device(of course, they still need to think of the appropriate placement and \textit{SBP} signatures for each tensor).

%Even though \SysName{} does not require the users to directly program with the various low-level communication primitives, 

%manually specifying placement and \textit{SBP} signatures seems to be still too complex for the developers to specify. 




==> motivation2.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figure/13-mem-schedule.eps}
    \vspace{-0.3cm}
    \caption{An example which may cause deadlock with the scheduler in existing frameworks.}
    \label{figure:graph_executor}
    \vspace{-0.6cm}
\end{figure}
%\jinhui{TODO: explain what is graph executor} 

\begin{figure*}
         \centering
         \includegraphics[width=1\linewidth]{figure/pipeline/02-01-oneflow_pipeline_long_train.eps}
     \vspace{-0.3cm}
     \caption{Pipelining of data-loading, pre-process, copyh2d and computation, where the computation is the bottleneck.}
     \label{figure:preprocess_pipeline}
    \vspace{-0.4cm}
\end{figure*}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{figure/08-tricky-allocator.eps}
%    \vspace{-0.2cm}
%    \caption{A customized allocator to support double buffering.}
%    \label{figure:allocator}
%    \vspace{-0.5cm}
%\end{figure}




%\vspace{-0.3cm}
\subsection{%Fatal 
Fundamental Flaws of the Existing Frameworks}\label{section:flaws} 
%\vspace{-0.4cm}

\subsubsection{Challenge of %dynamic
scheduling} 
In mainstream DL frameworks, %the scheduler is modelled as a graph executor. 
both \textit{data} and \textit{control} dependencies are represented with edges in the execution graph~\cite{abadi-2016-tensorflow, paszke-2019-pytorch, chen-2015-mxnet}. Upon completion of each op, the scheduler updates dependencies of the remaining ops and identifies ops who are ready to run (whose dependencies have all been resolved). Distributed DL can be more complicated in many scenarios due to the complexity of execution dependencies and resource management~\cite{rajbhandari-zero-2020, huang-2019-nips} (e.g., to avoid out-of-memory errors or deadlocks, to minimize the stalls, etc.). 

%The graph executor abstraction in traditional DL frameworks works fine for single-device and simple distributed training cases (e.g., \cwu{give example simple distributed training cases}).

Consider a simple example in Figure~\ref{figure:graph_executor}, %\cwu{Figure~\ref{figure:graph_executor} should be simplified without mentioning `acted' yet, and more intuitive}.
$M_{1}$ and $M_{2}$ are two data movement ops which serve two computing ops $O_{1}$ and $O_{2}$ on the same device, respectively. $O_{1}$ and $O_2$ do not depend on each other and $O_1$ requires more device memory to execute than $O_2$. $M_{1}$ and $M_{2}$ also require some device memory to store the output data. %The total amount of device memory is constant.
After $M_{1}$ and $M_{2}$ occupied their memory, % too much device memory, such that 
the free memory capacity can only satisfy the demand of $O_2$ but not those of $O_1$, while both $O_1$ and $O_2$ are in the ready set of the scheduler (as in TensorFlow's) at the same time.

$\bullet$ If $O_2$ is scheduled first, it can successfully execute and consume the output of $M_{2}$ in device memory. Once $O_2$ is done, the input and output of $O_{2}$ can be released, and $O_1$ can be accommodated, %the free memory may satisfy the requirement of $O_1$, 
which can then be executed.

$\bullet$ If $O_1$ is scheduled first, the memory is insufficient for $O_1$. If $O_1$ is dispatched to the OS thread on which the scheduler is running (i.e., the \textit{inline} execution in TensorFlow), the OS thread will be blocked. As a result, $O_{2}$ will never be scheduled even if the memory is sufficient for $O_2$.
Even if another OS thread is made to execute $O_{1}$, the framework still needs to handle the tricky issue of determining an appropriate number of threads for a dynamic thread pool, and implementing a customized memory allocator which supports complicated retrying mechanism.
%If the execution queue is empty at this moment, the blocking of $O_{1}$ will make the device be in idle.

%\hz{the footnote should be moved to the body, if used by tensorflow or other frameworks}


To avoid the second deadlock case while enabling the first case above, we need to perform static resource planning and specify an appropriate execution order in advance (e.g., adding \textit{control} dependencies between ops in TensorFlow). However, none of the existing frameworks has carried out static planning to avoid such deadlock risks. %, while relying on users to manually configure the dependency to avoid the case. 



\begin{figure*}
     \centering
     \begin{subfigure}[b]{1\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/pipeline/02-02-oneflow_pipeline_long_process.eps}
         \vspace{-0.8cm}
         \caption{Pre-processing bottleneck.}
         \label{figure:long_preproces}
     \end{subfigure}\\
     \begin{subfigure}[b]{1\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{figure/pipeline/02-01-oneflow_pipeline_long_train.eps}
         \vspace{-0.8cm}
         \caption{Computation bottleneck.}
         \label{figure:short_preprocess}
     \end{subfigure}
     \vspace{-0.3cm}
     \caption{An ideal pipelining for data-loading, pre-process, copyh2d and computation.}
     \label{figure:preprocess_pipeline}
\end{figure*}



%\vspace{-0.4cm}
%One way to address the deadlock issue is to increase the number of OS threads of the executor. Once the OS thread on $O_1$ is blocked, another OS thread can still execute $O_2$. However, determining the appropriate number of OS threads for a thread pool is another tricky issue: allocating too many OS threads introduces heavier context switch overhead; fewer OS threads may not resolve the bottleneck issue. Further, %not only the kernel scheduling becomes more tricky, but also the memory allocator becomes more complicated as well. For example in TensorFlow, the memory allocator supports a %type of
%retry policy which keeps retrying if an allocation request is not satisfied, %which further increases the 
%exaggerating unpredictability of the execution time needed by the operation. In distributed DL, the case is very complicated, since there are many data movement operations between devices and different nodes \cwu{ops? need to define what a node is referring to if using the term node}. \cwu{not sure if the pipelining mentioned below is the same as pipeline parallelism: if so, isn't tensorflow type of framework not supporting pipeline parallelism?pls clarify}

The case can become trickier if pipelining is in use. For example, each op may have multiple instances within a pipeline consisting of several consecutive ops, each corresponding to a different micro-batch at runtime. %parallelism, the data movement operations such as $M_{1}$ and $M_{2}$ may have multiple instances at run time. 
In state $\textcircled{2}$ of Figure~\ref{figure:graph_executor}, besides $O_{2}$, an additional $M_{1}$ or $M_{2}$ for the next micro-batch is ready to run. If the scheduler starts $M_{1}$ or $M_{2}$, they will consume part of or all the free memory. Then neither $O_{1}$ nor $O_{2}$ could execute successfully, and the outputs of the data movement ops thus cannot be consumed and be released. A deadlock results, and it is non-trivial to add control dependencies to circumvent this deadlock scenario. %\yuchen{I cannot understand the above sentence}
Further, when there are downstream operators of $O_{1}$ and $O_{2}$, specifying an execution order which allows successful execution of the entire program under the resource constraint is even more difficult.

Figure~\ref{figure:preprocess_pipeline} illustrates a pipelining for overlapping the data-loading, pre-processing, copyh2d (i.e., copy the data from the host memory to the device memory), and computation. The pipelining is implemented with the standard double buffering technique adopted by Nvidia DALI~\cite{nvidia-dali} and the dataset API in TensorFlow. As illustrated by the example, within the same batch, the downstream op depends on the upstream op (e.g., batch 6). However, when the pipelining enters the steady phase, the back-pressure enforces other ops to execute at the bottleneck op's pace (i.e., the computation). It leads to some counter-intuitive dependencies where the upstream op working on a new batch depends on a downstream op working on an old batch. For example, batch 4 of copyh2d depends on batch 2 of computation. Such pipelining effect is hard to accomplish by specifying execution order with control edges. Consequently, such pipelining is usually implemented outside the core graph executor of the existing frameworks~\cite{huang-2019-nips}.

%One may wonder whether it is possible to implement double buffering with the core mechanism of the existing frameworks. Figure~\ref{figure:allocator} illustrates a potential solution with TensorFlow. The idea is to implement a customized allocator which manages double buffers for each op. 

%$\bullet$ When an op \textit{allocate}s memory with the allocator, the allocator queries a counter whether the op has a free buffer to use. If so, it allocates a buffer to the op and lets the op proceed, and releases it after the op completes its computation. Otherwise, the allocator inserts the step $\{\textcircled{2}, \textcircled{3}\}$ into a waiting list.

%$\bullet$ When an op \textit{release}s its memory with the allocator, the allocator updates the counter of free buffers corresponding to the op, and checks whether there are ops in the waiting list depending on the buffer. If so, it pops the ready items from the waiting list and performs $\{\textcircled{2}, \textcircled{3}\}$. However, such implementation shows a bad practice of software engineering since it leaks part of the responsibility of a scheduler to the customized allocator.
%\hz{the detailed implementation of customized allocator is kind of off the topic. and I think the dependency tracking can be moved to the scheduler as well. the last argument doesn't hold water. if we want to keep this paragraph, better rephrase it, the current draft is hard to read}

%The framework just relies more heavily on pipelining to maximize the system throughput, which complicates the execution order further. \jinhui{Figure~\ref{figure:preprocess_pipeline} demonstrates it is hard to specify order in pipelining even with control edges. It turns out that allocating two registers to each actor suffices the requirement of pipelining for this specific case. The examples also demonstrate the effect of back-pressure. Since the computation is the bottleneck, and each actor has only two registers, the back-pressure mechanism enforces the other actors to execute  in the pace of the worker 4.}

%As demonstrated above, %by the above example,
%the actual execution order of operations in the graph executor of an existing DL framework (e.g., \cwu{point out it happens in which frameworks}) could be undetermined or quite random. It is therefore challenging to predict the execution time of a subgraph. However, predictability of execution time is a crucial prerequisite for effective scheduling of training tasks, e.g., in implementing pipeline parallelism, as arranging an appropriate execution order at runtime is too demanding for the executor. The DL framework has to statically analyze the resource constraints and the requirements of various operations while compiling a training job; in this way, the execution order of operations can be specified beforehand, to maximally eliminate the stall or the risk of deadlocks.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figure/14-data_movement_as_first.eps}
    \vspace{-0.3cm}
    \caption{The interaction between callback function and the scheduler.}
    \label{figure:data_movement}
    \vspace{-0.4cm}
\end{figure}

\subsubsection{Challenge in modeling data movement} 

%To make the graph executor work correctly, the graph executor must track all the dependencies for every operator. However, 

In existing DL frameworks, some dependencies between ops are not tracked by the scheduler. For example, TensorFlow only models inter-node data movements with \textit{Send} and \textit{Recv} ops in the dataflow graph, but does not treat data movement between a host and device memories as a normal op %nodes of
in the graph. Instead, it wraps such %non-networking
intra-node data movements in callback functions and inserts the callback functions where necessary. Figure~\ref{figure:data_movement} illustrates an example, in which $O_{2}$ is wrapped in a callback function which is expected to be invoked on the completion of $O_{1}$. However, if $O_{2}$ has other dependencies such as the output data of other ops or the \textit{control} dependencies inserted by the framework, the completion of $O_{1}$ does not necessarily suffice to resolve all the dependencies of $O_{1}$. To correctly and safely schedule $O_{2}$, the callback function should notify the completion of $O_{1}$ to the scheduler so that the scheduler updates all the dependencies of $O_{1}$. If the scheduler returns that all the dependencies have been resolved, $O_{2}$ can be scheduled immediately.  Otherwise, $O_{2}$ is inserted into a waiting list and will be scheduled in the future when other dependencies are resolved. 


%know whether all the dependencies of the inner operator are resolved, the callback function has to update and query the graph executor


%Such a callback function is triggered upon completion of an upstream operator, that \cwu{clarify what the upstream operator is}. \cwu{the following should be revised to clarify what the wrapped operator is and what the inner operator is referring to} 

%Note that, even the callback function is triggered, the wrapped operator may still not be ready to execute: triggering of the callback function may only due to resolving a single specific dependency; it is possible that other dependencies of the operator are still not resolved \cwu{give concrete example to show why this could happen}.

%to know whether all the dependencies of the inner operator are resolved, the callback function has to update and query the graph executor %\cwu{clarify what update it does to the graph executor}. 

%If the graph executor returns that all the dependencies have been resolved, the wrapped operator can be scheduled immediately; otherwise, the operator will be scheduled in the future when all other dependencies are resolved. 

If the callback functions are inserted manually by users like  Megatron-LM~\cite{mohanmmad-megatron-2020}, the framework has to expose the internal scheduler % \cwu{is it graph executor? unify the terminology}
to users. Only in this way can the user code correctly interact with the scheduler. Nevertheless, none of the existing DL frameworks expose the underlying scheduler %\cwu{is it graph executor? unify the terminology} 
to users yet. Therefore, the safety is not guaranteed for manually inserting callback functions.

In an alternative way to facilitate the above, %address these challenges, on the one hand, 
the scheduler needs to represent and manage all the dependencies for all the operations, without outliers. Substantial engineering efforts are required to modify the existing DL frameworks to ensure its completeness. First, the graph compiler should cover the computing ops as the traditional DL frameworks do, and include all the data movements as ops explicitly. Second, all the hard-coded callback functions inserted by the system need to be extracted from the runtime code and converted to normal ops managed by the scheduler.

%For example,  However, the design and implementation of the current DL frameworks cannot achieve this straightforwardly, if not impossible: on the one hand, the graph compiler should 
%besides the modification of the graph compiler, substantial engineering efforts are also required on the executor %\cwu{give more concretely what efforts are needed on the executor} 
%since the current implementation is largely for computation scheduling.% \jinhui{add a figure} 

%\subsubsection{Centralized scheduling is inefficient} %Suppose the framework not only models computation but also represents all the data movement in the dataflow graph. Hence the graph executor is able to track and manage all the dependencies. Let us think about how to efficiently implement the graph executor.
\subsubsection{Minimizing the runtime overhead in scheduler}

A microsecond-level overhead can also hurt system performance if it is on the critical path and frequently occurs~\cite{wang2019lineage}. A well-implemented generic DL framework must try its best to reduce the runtime overhead.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/15-02-threads-interaction.eps}
    \vspace{-0.2cm}
    \caption{Four threading models to implement a scheduler.}
    \label{figure:centralized}
    \vspace{-0.5cm}
\end{figure}

In existing DL frameworks, prohibiting the OS thread running the scheduler (i.e., the \textit{scheduling} thread) from performing expensive operations is a common wisdom. Given that the ops in the graph can be either computation or data movement, the execution of an op may take a while, and the actual operation is usually offloaded to accelerators such as GPGPUs or other worker threads. Suppose we allow the \textit{scheduling} thread asynchronously launches CUDA kernels (i.e., summarized as a  \textit{launching}). In that case, the \textit{scheduling} thread must set the corresponding device context before each invoking of low-level APIs on a particular device. 

Figure~\ref{figure:centralized} demonstrates several threading models for performing \textit{scheduling} and \textit{launching}.

$\bullet$ In case \textit{a}, using a single thread to manage the global state of the scheduler and serve several devices may frequently switch the device context, which has microsecond-level overhead. 

$\bullet$ In case \textit{b}, the \textit{scheduling} thread doesn't launch CUDA kernels directly. Instead, \textit{launching} operations are dispatched to some worker threads, each of which serves a particular device. In this case, the worker thread does not need to pay for the overhead of device context switching, but it suffers from the overhead of going through the scheduling thread as an intermediate proxy between two ops, since a single scheduling thread solely manages the global state of the scheduler.

$\bullet$ In case \textit{c}, to eliminate the proxy overhead in case \textit{b}, % caused by the extra hop on the centralized scheduling thread, 
we can create a pool of worker threads running the scheduler concurrently, the upstream and downstream ops on different worker threads directly talk to each other, and the global state of the scheduler must be protected by locks. It eliminates the extra hop through the scheduling thread but may increase the overhead of contention caused by concurrently accessing the shared state from multiple worker threads. However, a coarse-grained lock can severely hurt the overall performance. 

$\bullet$In case \textit{d}, to minimize the contention overhead in case \textit{c}, observing the states of the ops can be decoupled by op, fine-grained locks can be used (e.g., creating a dedicated lock for protecting the state of each op in DL scenario). The scheduler of TensorFlow belongs to such a category. However, it is tricky and error-prone while optimizing the program by reducing the scope of a lock.

We would like to find a better approach to leveraging the localized and decentralized state management of ops. On the other hand, the actor programming model~\cite{hewitt-ijcai-1973}, which represents a lightweight, independent execution unit with each actor encapsulating a local state, is widely used to construct massive, distributed systems~\cite{phillipp-2017-ray, paris-2015-flink, akka, bykov2011orleans, virding1996concurrent, charousset2013native}, and it proves to be very useful for decoupling and abstracting decentralized state management.
%and its states with a state machine. 
%\hz{which category does Tensorflow and others belong to?}

% synchronize with each other \cwu{clarify how this can avoid the extra hop}. A better idea is to enable each op to manage its state itself, in a decentralized manner \cwu{each op can manage its state, but what about state synchronization across ops? pls clarify.}. 



%Suppose all data movement ops are modeled in the dataflow graph. 
%If we limit the graph executor to running on a single OS thread (referred to as the scheduling thread), %to make the graph executor responsive enough, 
%we shall dispatch all the %actual work of the 
%op execution to worker threads other than the scheduling thread, as otherwise, the execution of ops may hinder timely update of other operators' dependencies by the graph executor. 

%Nonetheless, as shown in Figure~\ref{figure:centralized}, state synchronization between an upstream operator and a downstream operator residing on two different worker threads \cwu{clarify what the state synchronization is} has to %communicate with the help of
%go through the scheduling thread as an intermediate proxy, inevitably increasing the scheduling overhead. 



%\jinhui{add a figure}

%\jinhui{The above thought experiment also holds for the dynamic graph executor in PyTorch. Actually, the dynamic graph execution provides worse support to resource planning and \textit{ctrl} dependencies.}


%\jinhui{TODO: add a figure to explain the issue}
%\vspace{-0.5cm}
\subsection{Summary of Motivations and Design Overview}
In summary, we seek to implement a distributed training framework that achieves four goals: %\cwu{expand the following descriptions} 
(1) automatically programming the data routing in various parallelism by the framework instead of programming by hand; (2) safely handling implicit dependencies introduced by resource constraint; (3) elegantly scheduling data movement as a first-class citizen; (4) maximally reducing the runtime overhead in the scheduler. We achieve these goals through a holistic design from compiler to runtime. The compiler performs the static planning and generates an execution plan, while the runtime provides a flexible mechanism instantiating and running the compiled execution plan.  

%\cwu{need a paragraph of overview, stating that the system includes a compiler and a runtime, each for xxx purpose, etc.}
%\vspace{-0.4cm}

%xFlow does not have such a flaw. Firstly, the static resource allocation may limit the memory quota of data movement Ops at compile time to allow $O_a$ to execute. Secondly, resource readiness becomes part of the trigger condition of the actor hosting $O_a$. If the resource can not satisfy the requirement of $O_a$, the actor system just does not trigger $O_a$ (i.e., putting it into a ready set). Finally, no matter whether an Op is ready or not, it never blocks the OS thread.


%\begin{comment}

%\vspace{-0.4cm}
%\subsection{Managing the Kernel States}
%\vspace{-0.2cm}
%A discouraging fact of DL is that the overhead of its auxiliary operations is significant compared with the kernel execution time: 
%\textbf{The heavy runtime overhead} As a kernel of a distributed DL training usually takes only up to tens of milliseconds for either computation or data transfer, auxiliary tasks that consume tens or even hundreds of microseconds, such as device context switching, memory allocation, kernel launch and initialization, become non-negligible. Furthermore, to fully support asynchronous data transfers between host and device memory or leverage networking techniques like RDMA, the memory should be pinned or page-locked, which may also increase the overhead of auxiliary operations. Existing DL frameworks mitigate such overhead using approaches that can minimize the number of function invocations, e.g., dynamic memory pooling. In addition, caching the local device context is also used to reduce such overhead.

%, but they require long-lived kernels with attached dedicated resources.
 %Uncertainty may hurt the system efficiency and stability. 
%\vspace{-0.4cm}
%\paragraph{Runtime unpredictability} Existing DL frameworks attempt to allocate memory for the output tensor of a kernel when the kernel is issued by the kernel executor, which is in turn allowed to enter a ready queue provided its input data is available. The system returns an out-of-memory error or retries later when this memory allocation fails. This uncertain runtime behavior makes it difficult to predict the kernel execution time, aggravating the complexity of the kernel executor. Another scenario causing the unpredictability happens when mapping a kernel to an OS thread. A system usually allocates a thread pool using a fixed number of OS threads for parallel execution, but this may also introduce implicit dependencies between the kernels mapped to the same thread. Worse yet, mapping kernels to OS threads is a runtime, dynamic process, but the statically assigned number of OS threads may not be sufficient to fully exploit the parallelism degree of a given DL workload.


%\vspace{-0.4cm}
%\paragraph{Ineffective support of pipelining and flow control} Existing DL frameworks usually support the overlap between communications and computations using asynchronous callback functions. They leverage a chain of nested callback functions. The in-order execution of the nested callback functions, i.e., each callback function only executes after the body of its caller function is finished, is triggered only when a piece of input data is received. However, the chain of callbacks may receive multiple pieces of input data that are processed in divergent stages, which may lead to the overflow of the system resources without a congestion control mechanism. Imagine a case that one of the pipelined stages slows down due to unknown noises of the environment while its upstream stages proceed normally. The upstream stages will produce a large number of intermediate data and thus occupy much of the memory. The system will crash due to the out-of-memory error without a back-pressure mechanism. %To support back-pressure, the framework should provide a mechanism for describing and exchanging the states of kernel execution.


%\vspace{-0.4cm}
%\paragraph{Summary} We view both the dedicated resources attached to a kernel and those triggering conditions as the components of its state. A distributed DL framework should be able to isolate the state of a kernel from other unrelated factors for effective state management.
%need to provide a mechanism to abstract out the state and separate the complexity of state management from other concerns.
%\vspace{-0.4cm}
%\subsection{The Actor Model}
%\vspace{-0.2cm}
%\subsection{Opportunities of Actor Model in Deep Learning Framework}
%We propose to add a wrapper outside kernel to manage its state including dedicated resource, the mapping and binding relationships between kernel $\sim$ thread $\sim$ device and the constraints for the kernel execution. Based on our investigation, the actor model is helpful to achieve this goal because of its modularity and composability.



%By considering using actors as a generic abstraction to represent most of components in DNN training (e.g. computation, communication, input data loading, etc.), we find the actor framework can provide opportunities to efficiently expedite DNN training which is hard to achieve in existing training frameworks.

%\vspace{-0.5cm}
%\paragraph{Long-lived kernel with dedicated resources} Managing the kernel states using actors makes it straightforward to bind dedicated resources to a kernel, allowing for the long liveness of a kernel and the decrease of the frequency of device context switching and memory allocation. The actor model also makes it possible to estimate the size of dedicated resources for a kernel before running, avoiding the runtime unpredictability as introduced before.


%\vspace{-0.5cm}
%\paragraph{Fine-grained controls of the kernel execution} The state machine of an actor enables the state separation of a training task from other unrelated factors; it also provides a fine-grained managing mechanism for these states, thereby leveraging the stable resource consumption of DL training tasks and providing back-pressure required by flow control. 


%\vspace{-0.5cm}
%\paragraph{Native pipeline parallelism} As we introduced before, pipeline parallelism has to be enabled by hand in existing frameworks due to the passive mode of kernel invocation. A typical scenario in an existing framework is the excessive attention paid to optimize the sub-graph of internal computing primitives. While improving the performance, this approach has to develop additional customized data loading and pre-processing library for hiding communications behind computations~\cite{kumar2020exploring}. This makes the frequent data feeding the performance bottleneck, and one thus has to resort to external plugins such as Nvidia DALI~\cite{nvidia-dali} to optimize the pipeline. On the contrary, an actor prefers to handle a message as early as possible and performs its computation task in a network-based manner as long as all the required resources are available. The actor model fully automates the pipeline parallelism by executing the data loading and computation using individual actors.

%\noindent\textbf{Eliminate the bottleneck of loading training data.}Data parallelism is widely used for scaling DNN training over large datasets, but mainstream deep learning frameworks \cite{} usually pay most attention to optimize the intern computing primitives, not for the data layer, which is in charge of reading and preprocessing input data. Fundamentally current deep learning frameworks use a directed acyclic graph (DAG) model to describe different algorithms in different networks and then employ a set of system or graph optimize techniques to achieve fast training, for example, the data-parallel method. However, ignorance of data loading and preprocess means frameworks don't draw this into the computing graphs so that the whole data input procedure will not be taken into consideration when optimizing or overlapping with other computing. It has exactly become the system bottleneck when input data is extremely increasing in amounts \cwu{need  concrete example} . Hence it could be easily inferred that properly preprocessing input data will achieve expediting distributed DNN training performance if the data-parallel method works. However, with the actor model, the process of loading data and following computation can be assigned to different actors and be naturally executed in an efficient pipeline manner.

%\noindent\textbf{Reduce uncertainty at runtime. }Estimating the optimal parallelism degree for each DL workload and statically binding the kernel to specific thread help the eliminate uncertainty at runtime.

%\noindent\textbf{Simplify the data movement logic.}
%Distinguished from existing frameworks and libraries relying on special operators Send and Recv to stitching subgraph execution on different nodes, networking actors can be inserted into the system automatically \cwu{not clear how it is different from having Send and Recv ops}. At runtime, the networking actor receives \textit{message} notifying the readiness of \textit{registers} to receive data%\cwu{no any definition or explanation of registers before this point}
%. Then the networking \textit{actor} will start reading the remote data via RDMA or socket to make a local copy so that the downstream \textit{actors} always read locally.
%This mechanism is totally transparent to the end users, which enables them to scale a model from one node to thousands of nodes without writing any imperative code to move data.

%\noindent\textbf{Good scalability with decentralized scheduling.} With the actor model in \SysName, there is no single central scheduling node because each \textit{actor} is only concerned with the upstream actors producing the data it consumes and the downstream actors consuming the data it produces. Due to this nature of event localism, there is no overhead of message round-trip. When it comes to large scale distributed training, the scheduling bottleneck points inherent in central scheduling systems are absent in \SysName. \cwu{if scheduling is done just once before running, it does not matter to be centralized. Here we may emphasize online training hence online scheduling.}\jinhui{There is still scheduling at runtime. In centralized scheduling, each worker report its state or progress to the executor, which makes decisions according to the collected information and drive the other workers to run. In decentralized scheduling, the workers directly communicate with each other if necessary, thus eliminating the the intermediate proxy (i.e., the centralized executor).}


%\vspace{-0.4cm}
%\subsection{Challenges}
%\vspace{-0.2cm}
%While the actor model provides a large number of optimization opportunities for designing a distributed DL framework, it also brings some challenges: (1) how can we make the framework concise and general? (2) how can we generate effective execution plans for actors along both spatial and temporal dimensions? (3) how can we minimize the overhead of the actor-based framework?  These challenges will be addressed in the following context by modeling the various components of a distributed DL framework in a unified actor abstraction.

%\end{comment}

%\begin{comment}


%\noindent\textbf{How to distill an abstraction which is highly concise but general enough to serve the purpose of distributed DL? } The actor concept must unify the common characteristic of all types of operations, including both computation and various data routing in distributed DL. The protocol between actors must be general enough to specify how the actors interact with each other in various scenarios. 


%\noindent\textbf{How to automatically generate the execution plan for scheduling actors in both spatial and temporal dimensions?} Given a neural network described by a logical graph and a dedicated set of devices, the framework is expected to automate the generation of the physical graph, no matter what type of parallelism policy is used. The physical graph acting as an execution plan characterizes the topology of actor interaction and specifies the behavior and the resource quota of each actor.

%\noindent\textbf{How to reduce the overhead of the actor based system?} Since DNN models usually consist of thousands of operations, the amount of actors to manage these operations is also large, which may cause serious overhead in the aspect of resource race condition, thread scheduling, device context switch, etc. in the system without carefully designed optimization methods.

%\end{comment}

%\noindent\textbf{What if ``congestion'' happens in the actor-based system?} Since the actors actively and asynchronously do execution in a network manner, there might be situations that some actors are not able to consume input data in time, resulting in increasingly accumulated input data. Similar to the network congestion, this situation may lead to extremely poor performance of the DNN training.

%\noindent\textbf{How to describe DNN models with different kinds of parallelism strategy candidates?} For different type of operations, they may have different kinds of available parallelism strategies, without knowing these features, it is hard for the system to build an efficient distributed strategy for the DNN training. 



%\vspace{-0.3cm}
%\subsection{\SysName~Overview}
%\vspace{-0.2cm}
%\SysName~works with the following essential operations. At compile time, user-defined neural networks and distributed environment configurations are fed into the \textit{compiler}. After conducting a series of analyses and optimizations, the \textit{compiler} will generate a \textit{plan}, which is a graph describing the execution and computation of neural networks. A single \textit{actor} corresponds to one node in the \textit{plan}. While an edge represents a \textit{register}, which holds memory addresses an \textit{actor} can use. At runtime, each node in the user-defined distributed environment configurations initializes local actors according to the \textit{actor} definition in the \textit{plan} and starts the actor system.

==> outline.tex <==
\section{Todo and Owner}
%-------------------------------------------------------------------------------

\begin{itemize}
    \item Introduction (1 page, draft by jinhui). Why do we need a top-down design of distributed deep learning framework?
    \item Problem description (1 page, draft by jinhui). The logical structure, hardware foundation, the streaming workload and complicated dependencies of distributed deep learning job.
    \item Break-down of training cost (1 page, draft by jinhui). Computation, data movement, scheduling cost, runtime overhead.
    \item The Challenges of Data Movement (1 page, draft by jinhui). Overlapping data movement and computation, flow control, etc.
    \item The Complexity of Scheduling (1 page, draft by jinhui). Placement, parallelism, memory planning, dependency management, we have to move the scheduling cost to compile time.
    \item SBP Infrastructure for Static Scheduling (2 pages, fei yang and yipeng). It should provide infrastructure for automatically infer the optimal placement, parallelism policy. Meanwhile, it should provide mechanism for automatically map the optimal policy to execution plan with correctness guarantee.
    \item Extremely Light-weight Actor System (2 pages, by shenghang, haijun, zhejiang).
    \item Implementation.
    \item Case Study. (1 page for each case) 1. data pre-processing pipelining in data parallelism, nvidia dali. 2. model parallelism, insightface, deep and wide. 3. pipelining  parallelism, gpipe, pipedream. 4.hybrid parallelism, GPT.
    \item Evaluation. (we may merge the content of Case Study and Evaluation. In each case, we provide its implementation in \sys{} and performance evaluation)
    \item Conclusion.
\end{itemize}

\section{Outline}

\subsection{Introduction}

Through learning the representations of training data, deep learning proves to be the state of the art approach in various real-world applications. 

computation increase. resnet, bert. gpt. leveraging the weakly supervised data; increasing the number of prameters; automl, learning the optimal structure of neural networks. The number of computations, eflops. 

a modern accelerator, V100, A100's capability, with a single accelerator, it requires dozens of months. 

the computation limitations of hardware.

To reduce the training time, an alternative is to leverage distributed computation. With the help of algorithmic trick of enlarging the batch size (LARS), accelerators, distributed deep learning framework, some specific training task which previously requires days of computation can be completed in a minute.
(cite mlperf) 

However, solving the general scaling out problem is a crucial, common challenge. The focus of a deep learning framework running on a single device and that running on distributed cluster is different. Distributed deep learning has introduced some intrinsic complexity. (comparison between single device and multiple devices)

difficult to efficiently train, utilization (TODO examples, not efficient)

each specific solution is complicated (TODO examples, not concise)

the techniques specific to niche needs, multiple proposals co-exist (TODO examples, not general) 

the goal of this paper, is it possible to create a minimalist design of distributed deep learning framework, simple yet correct, efficient, general to a broad requirements.



the SBP abstraction.
the optimal parallelism
the actor runtime mechanism.


\begin{itemize}
    \item distributed deep learning is crucial. We need an efficient, concise, general abstraction.
    \item the essential challenges
    \item static scheduling (placement, parallelism, routering)
    \item zero run-time overhead
    \item derive an abstraction to serve static scheduling (SBP), zero-runtime (actor)
\end{itemize}

With a Deep neural networks learns and represents the statistical patterns underlying the data.

to summarize and highlight the challenges of distributed deep learning.


correctness, programmability and efficiency.

in this paper, we don't discuss the issue of eager mode. assume the static graph.

simplicity 
\begin{itemize}
    \item is it possible to unify the whole system? in existing frameworks, only the computation is modelled in graph executor. Is it possible to unify data movement and computation? especially the networking? let's make everything an operator, either moving data or transform data, make everything a node (operator) of the graph.
    \item in existing frameworks, the data movement is usually outside the graph executor, nesting of callback function.
    \item separation of concern. an operator is managed by an actor, finite state machine, the message passing.
    \item let the topology of the actor network be programmable
    \item let the behavior of each actor be programmable
    \item let the schedule can be optimized (compiled)
\end{itemize}

the benefits of abstraction. the power of abstraction
\begin{itemize}
    \item correctness
    \item simplicity
    \item generalization
    \item efficiency
\end{itemize}

implementing a novel distributed system, it is developed in the past 4 years, the whole history can be tracked in GitHub. 

given the various constraints, find the minimal, precise, simple abstraction.

bottom up and top down design
occam's razor, we are curious about what is the minimal design of a distributed deep learning framework to maximally satisfy the various complicated requirements. 


\subsection{Motivation}

the hardware abstraction, the array of accelerators, neglecting the nonuniform topology. each accelerator has a limited capacity of memory which the accelerator could efficiently access. A common case is the bandwidth between accelerators may be one or two order of magnitude lower than the internal bandwidth of an accelerator. (draw figure). the reality (nonuniform topology, limited memory capacity)

the complicated dependencies, the non-unidirectional dependency. the algorithmic abstraction, DAG, the unusual feature of the DAG in deep learning is that it involves a forward and backward pass. (draw a figure). 

the streaming workload, tiny granularity. each batch of incoming data may incur an update of internal state, which may trigger global state synchronization if the state is distributed. millions of transient tasks, a kernel may only cost a millisecond, a forward pass may cost tens of milliseconds. 



to maximize the throughput, we have to consider the locality issue, load-balance, the allocation of computing, memory, bandwidth resource.

the basic ideas

the hypothesis space of deep learning system, constrained from two direction, top down and bottom up. The algorithm assumptions (basically dense computation) and hardware (accelerators and servers, RDMA networks).

the challenges of distributed deep learning. 

the efforts to accelerate the computation on a single device

\begin{itemize}
    \item logical computation
    \item hardware basis
    \item algorithm, streaming
    \item the implication
\end{itemize}

\begin{itemize}
    \item inference framework, kernel fusion
    \item deep learning compilers (mlir, onnx, onnx-runtime)
    \item autotuner, automatically figure out the optimal hyperparameters
\end{itemize}

what lessons we can learn from previous work.

why static? make the scheduling policy as static as possible (add some experimental result)
the typical communication cost; the kernel launch cost; the average kernel running time; the resource allocation time. 

(measure the time with raw framework, without caching, the existing framework usually overcomes the problem with cache, why not direct hard-code the scheduling policy)

the historical lessons (static scheduling, VLIW, Rammer etc)

based on the observation, we derive some constraints (as static as possible). we have to make the system as static as possible, the static analysis involves placement, parallelism etc.

optimally mapping the logical computation to physical devices is difficult (cite google's paper). However, a significant choice of deep learning is the so-called static placement. 

(dynamic placement is almost impossible) 
scheduling overhead and data movement cost are non-negligible.

minimize the data transfer.
static policy makes the problem predictable, pre-send or pre-fetch is possible.

deep learning is repetitive. it is possible to make the scheduling as static as possible.

placement and parallelism is twisted together. we assume the placement is solved. 

there exists a few choices (draw a figure), a naive placement versus a pipelining placement. where the computation task is placed.

given a placement policy, it introduces the parallelization problem.  (draw a figure, given some examples), an operator has its optimal parallism choice. it also depends on its context.

given a parallelism policy, there exists a corresponding data routering policy. How to correctly and efficiently implement the routering infrastructure?

provide an infrastructure to support automatically searching the optimal placement, parallelism policy, support the data routering.

support memory planning, pipelining etc. minimize the runtime-overhead. the flow control etc.

the minimalist design of distributed deep learning framework must provide the necessary infrastructure for automatic static scheduling, meanwhile, the minimal runtime overhead (Amdahl's law).

\begin{itemize}
    \item the description of deep learning algorithm and hardware settings
    \item the SGD algorithm and GPGPU, TPU and other accelerators.
\end{itemize}



Yet another deep learning framework

lessons learned in data parallelization

\begin{itemize}
    \item SGD, streaming workload, increase the batch size, LARS and LAMB, without increasing the number of devices, larger batch means lower frequent parameter synchronization such as Allreduce
    \item Data preprocessing pipelining, overlap the data preprocessing with the computation DALI
    \item Allreduce, ring allreduce, double tree, bytePS, Horovod, 2D torus allreduce, 
    \item Overlapping forward, backward and variable synchronization and optimizer (bytescheduler improves the communication in model updating)
\end{itemize}

the challenges of extremely large model

\begin{itemize}
    \item face recognition, deep and wide, Nvidia MegatronLM, Microsoft Turing, OpenAI GPT-3
    \item sublinear memory allocation, Microsoft ZeRo and deepspeed
    \item mesh-tensorflow, gpipe, gshard.  Zhihao Jia, Huawei Mindspore
\end{itemize}

what new stuff \sys{} can contribute to the community?

the dataflow description of deep learning algorithm, the operator and tensor, following the conventions of tensorflow.

\begin{itemize}
    \item the correctness issue, it is challenging to correctly implement a model parallelism of deep learning model. (with SBP abstraction)
    \item the implementation complexity (the pipelining, the single device compilation, the communication, the memory management, the resource allocation, with an actor abstraction)
    \item the runtime efficiency (runtime overhead, the static scheduling)
\end{itemize}

build a concise, correct, simple, minimal and efficient system.

characteristics of distributed deep learning.
\begin{itemize}
    \item streaming workload, stochastic gradient descent algorithm
    \item heterogeneous computation, accelerators.
    \item in the result, millions of transient tasks in a second.
    \item how to minimize the runtime overhead?
\end{itemize}

separation of concern. 

\begin{itemize}
    \item lessons learnt from data-parallelism, model-parallelism, pipeline parallelism.
    \item complex parallelism pattern. 
    \item hard to program. separation of concern
    \item hard to ensure the correctness
    \item hard to guarantee the efficiency.
\end{itemize}

\begin{itemize}
    \item overlapping data movement and computation is crucial. involving complex interleaving data movement and computation. such as data-preprocessing and training (the merit of DALI), the overlapping of forward, backward pass and Allreduce; the overlapping of data movement in pipelining parallelism. 
    \item minimize the runtime overhead, especially resource allocation. with the repetitive and predictable pattern in mind, to reduce runtime overhead, a typical way is caching. Push it forward further, make it as static as possible.
    \item manage the complicated dependencies. data dependencies, control dependencies, resource dependencies which are usually not explicitly described, which is delegated to runtime system. 
\end{itemize}

\subsubsection{Static Scheduling}

a minimal abstraction of distributed deep learning framework.

make the system as static as possible, reduce randomness

lessons learned from inference engine, static memory allocation plan, instead of memory pool.

compiler (iree, grapler)
\begin{itemize}
    \item auto-placement
    \item auto-parallelim
    \item the memory planning (XLA static memory planning)
    \item the computation resource binding (thread, stream)
    \item the bandwidth planning
    \item software pipelining (flow control)
\end{itemize}



\subsection{SBP Formulation}

the mathematical abstraction of parallelization. the abstraction ease the programmability of deep learning algorithms (separating the algorithmic description and placement, the default placement, the default parallelization), meanwhile provide the support for compile stage, especially the auto-parallelization.

\begin{itemize}
    \item the correctness.
    \item mathematical abstraction of parallelization (SBP) on numpy operation (GShard paper)
    \item the deduction rule (2D SBP, spatial and temporal shape)
    \item the backward direction SBP
    \item the transition between two operators in succession (boxing, reducescatter, allgather, all2all, one2one
    \item cost model and auto-parallel approach (Zhihao Jia's paper)
\end{itemize}

\subsection{Actor System}

\subsection{Case Study and Evaluation}

\subsection{Summary}






==> related.tex <==
%\vspace{-0.3cm}
\section{Related Work}


%\vspace{-0.3cm}
%\subsection{DL Frameworks and Compilers}
%\vspace{-0.2cm}
%To simplify the implementation of various DL models, several popular DL frameworks have been proposed such as TensorFlow \cite{abadi-2016-tensorflow}, PyTorch \cite{paszke-2019-pytorch}, MXNet \cite{chen-2015-mxnet} and Chainer \cite{tokui-2019-chainer}. However, most of these training frameworks do not support model parallelism, pipeline-parallelism natively.
%are initially designed for single-device training, or supporting simple data parallelism without carefully considering the overhead of data movement between devices and complicated parallelism strategies.
%\subsection{Deep Learning Compilers}
%To alleviate the burden of optimizing the DL models on each DL hardware manually, several popular DL compilers have been proposed such as TVM \cite{chen2018tvm}, Tensor Comprehension \cite{vasilache2018tensor}, Glow \cite{rotem-2019-glow}, nGraph \cite{cyphers2018intel}, XLA \cite{leary2017xla}, MLIR~\cite{lattner-2020-mlir},Tiramisu~\cite{baghdali-2019-cgo} and Rammer~\cite{ma-osdi-2020}. The DL compilers take the model definitions described in the DL frameworks as inputs and generate efficient code implementations on various DL hardwares as outputs. The transformation between model definitions and specific code implementations is highly optimized, targeting the model specifications and hardware architectures. Currently, these works mainly focus on accelerating computation on a single device.

%\vspace{-0.3cm}
%\subsection{Parallel Strategies in Distributed Training}
%\vspace{-0.3cm}
%To support more complicated parallelism strategies, many schemes are proposed as wrappers or plugins based on some mainstream DL frameworks such as TensorFlow and PyTorch. Mesh-TensorFlow \cite{shazeer-2018-nips}, FlexFlow \cite{jia-2019-sysml} and GShard \cite{dmitry-2020-gshard} provide APIs for developers to express a wide range of parallel computation patterns for different components of DNN models. Among the existing work, GShard is most similar to the SBP abstraction proposed in this paper. The fundamental differences between the \textit{SBP} with the abstraction in GShard are discussed in Section \ref{sec:sbp}.
%\footnote{We develop \SysName{} with the SBP abstraction before we are aware of the Gshard paper. Just soon after Gshard is published, \SysName{} is open sourced at GitHub.}
%Horovod~\cite{alexander-2018-horovod} achieves efficient data parallelism in a homogeneous environment with highly-optimized collective communication library NCCL \cite{jeaugey2017nccl}. Stanza \cite{wu2018stanza} and DLPlacer \cite{pal2019optimizing} adopt data parallelism for training convolutional layers in CNN models and model parallelism for other layers. OptCNN \cite{jia-2018-icml} parallelizes CNN model training by splitting operations along batch and channel dimensions on homogeneous devices. Tofu \cite{wang-2019-eurosys} utilizes a partition-n-reduce method to split a single operation into sub-operations and a dynamic programming approach to optimize the partition recursively; no device placement of operations is considered. FlexFlow \cite{jia-2019-sysml} explores the SOAP (Sample-OperationAttribute-Parameter) search space to address parallelism within and across operations. HeteroG \cite{yi2020optimizing}, Placeto \cite{addanki2018placeto} and GDP \cite{zhou2019gdp} utilize Graph Neural Network and reinforcement learning to produce efficient distributed strategies for various DNNs.

%Pipelining has been studied to accelerate DNN training: different DNN layers are deployed on different devices; a mini-batch is divided into micro-batches. The micro-batches can be processed at different devices concurrently. GPipe \cite{huang-2019-nips} uses pipelining to address memory bottlenecks for training large DNNs. PipeDream \cite{narayanan-2019-sosp} introduces a pipelining approach to overlap communication and computation for asynchronous training. HetPipe \cite{hetpipe} integrates pipeline parallelism with data parallelism in a heterogeneous environment, making layer-based parallelism decisions. These pipelining strategies are all based on existing frameworks such as TensorFlow. Large amounts of sub-operations and control dependencies need to be added to the computation graph to achieve an efficient pipeline by DNN developers themselves. 

%As we mentioned, most of these works are based on existing training frameworks that are not dedicated to such complicated parallelism strategies, which yields both great engineering efforts and non-negligible system overhead. 

%GPT-3~\cite{brown-gpt-2020}

%Scaling laws~\cite{kaplan-scaling-2020}

%swapadvisor~\cite{huang-swapadvisor-2020}

%aibox~\cite{zhao-aibox-2020}

%checkmate~\cite{jain-checkmate-2020}

%\jinhui{test}

==> software_pipeline.tex <==
\vspace{-0.4cm}
\section{Finding the Optimal Register Number}
\vspace{-0.2cm}
%\jinhui{Yipeng, please write the flow control approach here, cite the paper \cite{allan-acmsurvey-1996}}
%\yipeng{Sure}
%\yipeng{TODO: might need to add sec in ref of section and tab in ref of table}
\SysName{} pre-allocates a fixed number of registers for each actor. Properly distributing memory to the stages in a pipeline is crucial for the actual system throughput. We address this challenge with the help of software pipelining technique \cite{allan-acmsurvey-1996}.

%For efficiency and avoiding running out of memory, our system pre-allocate memory for all execution units with static placement. For pipeline parallelism, it is a challenge to distribute memory for execution units properly with limited memory resources while keeping high computation resource usage. In this work, we address this challenge by introducing a flow controlling algorithm in our actor system.

Suppose the entire computation graph is divided into $n$ stages, each of which contains a set of consecutive operators. And a pipeline is deployed on $M$ GPUs. Denote the memory amount required by the $i$-th stage on GPU $k$ per execution by $m_{ik}$, the number of registers assigned to the $i$-th stage by $c_{i}$ and memory capacity of GPU $k$ by $r_{k}$, we have the following linear inequality system:
\vspace{-0.3cm}
\begin{equation}\label{eqn:limited resources}
    \sum_{i=1}^{n} c_{i}m_{ik} \leq r_{k}, \forall 1\leq k \leq M.
    \vspace{-0.3cm}
\end{equation}
Define execution time of the $i$-th stage $e_{i}$ to be the summary of execution time during forward and backward propagation, both of which can be estimated with an experimentally run. Then the lifetime of an register at the $i$-th stage is:
\vspace{-0.3cm}
\begin{equation}
    l_{i}=e_{i}+\left\{
    \begin{array}{cl}
        0 & \text{if } DS_{i}=\emptyset, \\
        \max_{k\in DS_{i}} l_{k} & \text{if } DS_{i} \neq \emptyset,
    \end{array}
    \right.
    \vspace{-0.3cm}
\end{equation}
where $DS_{i}$ is the set of all the downstream stages of stage $i$. The above recursive formula essentially calculates a longest path in the graph which depends on the registers at the $i$-th stage.

To estimate the required number of registers, we need to know the delay between the initiation of iterations of each new loop $II$, termed $\textit{initiation interval}$ in \cite{allan-acmsurvey-1996}.
%, under the memory capacity constraint of each device characterized in Equation %(\ref{equation:memory_contraint}). 
The smaller an initiation interval is, the faster the software pipelining will run. In an optimal pipelining, during the lifetime of a register, stage $i$ performs $\lceil \frac{l_{i}}{II} \rceil$ times of execution, which gives an lower bound of $c_{i}$ as
\vspace{-0.1cm}
\begin{equation}
    c_{i} \geq \frac{l_{i}}{II}, \forall 1\leq i \leq n.
    \label{equation:ii_constraint}
    \vspace{-0.1cm}
\end{equation}
For a given $II$, $c_{i}=\lceil \frac{l_{i}}{II} \rceil$ since GPUs will release the memory
of a register at the end of its lifetime. We find the minimum $II$ satisfying the constraints in Equation (\ref{eqn:limited resources}) and Equation (\ref{equation:ii_constraint}) with a binary search procedure. The lower bound depends on the longest run of all the stages,  
\vspace{-0.1cm}
\begin{equation}\label{eqn:ei II condition}
    II \geq \max_{1\leq i \leq n}\{e_{i}\}.
    \vspace{-0.1cm}
\end{equation}
An obvious upper bound can be obtained as the total time of an iteration. Once fixing $II$, we let $c_{i} = \lceil \frac{l_{i}}{II} \rceil$ accordingly, which decides a sufficiently optimal number of registers for the particular stage in software pipelining. 


%According to section \ref{sec:support pipeline and parallel}, each stage requires multiple memory blocks, or registers, to support pipelining.

%Theoretically, equations (\ref{eqn:limited resources}) (\ref{eqn:ei II condition}) (\ref{eqn:li II condition}) give us an lower bound of $II$. However, we might not be able to reach that in practice. \SysName{} use binary search with experimentally test to locate $II$ in interval $[ \max_{1\leq i \leq n}\{e_{i}\}, \max_{1\leq i \leq n}\{l_{i}\} ]$. We choose the right half of an interval for $II$ if GPUs runs out of memory.

%After fixing $II$, we fix $c_{i} = \lceil \frac{l_{i}}{II} \rceil$ accordingly, which decides a optimal static placement plan for software pipelining. 

%\yipeng{Should we add the following sentence?}
%\yipeng{There is an upper bound $\max_{1\leq i \leq n}\{l_{i}\}$ for $II$, which means we do not start any new iteration before we release the memory for all the registers.}
